TailCoR

Economic and financial crises are characterised by unusually large events. These tail events co-move because of linear and/or nonlinear dependencies. We introduce TailCoR, a metric that combines (and disentangles) these linear and non-linear dependencies. TailCoR between two variables is based on the tail inter quantile range of a simple projection. It is dimension-free, it performs well in small samples, and no optimisations are needed.

==> RV_Application_JoE.tex <==
\section{TailCoR of 21 financial
market indexes around the globe}

We illustrate TailCoR with an application to 20.5 years of daily stock log returns of 21 major equity market indexes that represent three geographical regions: America (S\&P500,NASDAQ, TSX, Merval, Bovespa and IPC), Europe (AEX, ATX, FTSE, DAX, CAC40, SMI and MIB), and East Asia and Oceania (HgSg, Nikkei, StrTim, SSEC, BSE, KLSE, KOSPI and AllOrd). The sample spans from 5 January 2000 to 9 July 2020 (each series contains 5369 observations). Table \ref{tab:returns} shows the countries and descriptive statistics. All medians are approximately zero, as expected.

The IQRs are a measure of volatility. If annualised, the maximum is Merval with 35\% and the minimum is KSLE with 12\%.
%{\color{red} percentage of what? of volatility? not clear to me}
European markets have annualised IQRs between 24\% for MIB and 17.8\% for SMI, while the IQR for S\&P500 is 16.5\%, very close to 15\%, the average that market participants consider as the average annualized volatility. All skewness are negative (but one albeit very close to zero) which indicates that the probability distribution is symmetric or very close to it. Finally, excess kurtosis are all positive, denoting tails heavier than Gaussian.  The open and international markets have the highest excess kurtosis -- the top 5 indices are in the US, South Korea, Netherlands and Canada.


\begin{table}
\begin{center}
\caption{Descriptive statistics} \label{tab:returns}
\begin{tabular}{cccccc}
 \hline\hline
Index & Country & Median & $\text{IQR}_{0.75}$ & Kurtosis & Skewness \\   \hline
S\&P & US & 0.0006 &  0.0104 &  1.8598 & -0.0034 \\ 
  NASDAQ & US &  0.0009 &  0.0137 &  1.9299 & -0.0036 \\ 
  TSX &  Canada & 0.0007 &  0.0098 &  1.6225 & -0.0042 \\ 
  Merval & Argentina & 0.0013 &  0.0221 &  1.4193 &  0.0008 \\ 
  Bovespa & Brazil &  0.0009 &  0.0200 &  0.5942 & -0.0029 \\ 
  IPC &  Mexico & 0.0006 &  0.0126 &  1.1945 & -0.0020 \\ 
  AEX & Netherlands & 0.0006 &  0.0126 &  1.6462 & -0.0036 \\ 
  ATX & Austria & 0.0007 &  0.0141 &  1.3296 & -0.0053 \\ 
  FTSE & UK & 0.0005 &  0.0113 &  1.4377 & -0.0028 \\ 
  DAX & Germany & 0.0008 &  0.0143 &  1.3958 & -0.0055 \\ 
  CAC & France & 0.0004 &  0.0138 &  1.3717 & -0.0038 \\ 
  SMI & Spain & 0.0006 &  0.0112 &  1.2319 & -0.0035 \\ 
  MIB & Italy & 0.0007 &  0.0151 &  1.2464 & -0.0038 \\ 
  HgSg & Hong Kong & 0.0006 &  0.0142 &  1.2157 & -0.0025 \\ 
  Nikkei & Japan &  0.0006 &  0.0155 &  0.9529 & -0.0030 \\ 
  StrTim & Singapore &  0.0002 &  0.0106 &  1.5006 & -0.0036 \\ 
  SSEC & China &  0.0008 &  0.0144 &  1.5891 & -0.0050 \\ 
  BSE &  India & 0.0009 &  0.0140 &  1.4791 & -0.0045 \\ 
  KLSE & Malaysia &  0.0004 &  0.0077 &  1.4068 & -0.0012 \\ 
  KOSPI & South Korea & 0.0006 &  0.0134 &  1.8703 & -0.0036 \\ 
  AllOrd & Australia & 0.0007 &  0.0096 &  1.1289 & -0.0034 \\ 
   \hline \hline 
\multicolumn{6}{p{11.5cm}}{\footnotesize{All the metrics are quantile-based. $\mbox{IQR}_{75}$ is the interquartile range, kurtosis is in excess and computed as $\mbox{IQR}^{0.975}/\mbox{IQR}^{0.75} - 2.91$, and skewness is computed as $(Q^{0.975}-Q^{0.50})-(Q^{0.50}-Q^{0.025})$.}}
\end{tabular}
\end{center}
\end{table}

%We illustrate TailCoR with an application to 10 years of daily returns of eight major US banks: Bank of America (BAC), Bank of New York (BK), Citigroup (C), Goldman Sachs (GS), JP Morgan (JPM), Morgan Stanley (MS), Wells Fargo (WFC), and State Street (STT). The sample starts in January 2, 2003 and ends in December 31, 2012.
% consists of 2517 observations. The initial date is January 2, 2003 and the ending date is December 31, 2012.

%\begin{center}[TABLE \ref{tab:returns} ABOUT HERE]\end{center}

%Table \ref{tab:returns} shows descriptive statistics. All the metrics are quantile-based. The column kurtosis is a measure of excess kurtosis, computed as $\mbox{IQR}^{0.975}/\mbox{IQR}^{0.75} - 2.91$. The skewness is computed as $(Q^{0.975}-Q^{0.50})-(Q^{0.50}-Q^{0.025})$. Visual inspection -- not shown here -- reveals strong volatility clustering, which is a conditional feature that may distort the unconditional measurement of the tails and their correlations. To safeguard against it, we adjust the returns with a GARCH(1,1).
%Once volatility clustering is removed, kurtosis diminishes but is always far from Gaussianity, as shown in the bottom panel of Table \ref{tab:returns}.
%The table shows that the adjusted returns share the stylized facts of financial returns: zero medians, a great deal of fat tails, and they are approximately symmetric.\footnote{We also did the analysis without the GARCH adjustment. Results are very similar because of the standardization (\ref{eq:standard}).}

We first show full-sample results, followed by rolling window estimations to study the dynamic behaviour. The window has a size of 3 years and it is rolled every year, i.e. we start with January 2000 - December 2002, followed by January 2001 - December 2003, and so on and so forth. There are between 780 and 800 observations per window (except the last one that ends in July 2020). The choice of 3 years is motivated by having a relatively small sample size (so we can compare the performance with the much larger full sample) but not too small (that would not allow us to draw meaningful comparisons with alternative measures).

Indeed, we compare TailCoR with the upper and lower exceedance correlations of \cite{LonginSolnik2001} (denoted $\theta^+(>\xi)$ and $\theta^-(<\xi)$, respectively), and the parametric and non-parametric tail dependence coefficients (the former with a $t$-copula and the latter as in \cite{Straetmans08}).\footnote{The non-parametric tail dependence coefficient is also called the co-exceedance probability; see equation (10) in \cite{Straetmans08}.} We denote them $\tau_p$ and $\tau_{np}$, respectively. Results are for $\xi=0.975$ ($\xi=0.025$ for downside correlation). Estimations for other values of $\xi$ are available upon request.\footnote{Since $\tau_{np}$ depends on the Hill statistic, alternative methods for choosing $\xi$ are available. See \cite{DIV16} for a survey.}

\begin{figure}
  \caption{Full sample results -- TailCoR and components}\label{fig:tailcor}
  \begin{center}
    \subfloat[TailCoR]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{TailCor}}
    \subfloat[Linear component]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{Linearcomp}} \\
    \subfloat[Nonlinear component]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{Nonlinearcomp}} \\
\begin{tabular}{p{13cm}}
%\scriptsize Heat maps for TailCoR and its components. The colour grading depends on the scale\\ 
\end{tabular}
  \end{center}
\end{figure}

%The upper panel of 

Full sample results are found in Tables \ref{tab:tailcor} to \ref{tab:nonlinearComponent} for TailCoR and its components (numbers in parenthesis are standard deviations multiplied by 100 for facilitating interpretation), and Tables \ref{tab:dexceedance} to \ref{tab:non-param} show results for $\theta^+(>\xi)$, $\theta^-(<\xi)$, $\tau_p$, and $\tau_{np}$ (the rightmost column in every matrix shows the row averages). These tables are lengthy and relegated to Appendix T. Figures \ref{fig:tailcor} and \ref{fig:competing} show a summary in the form of heat maps. The market indexes are ordered as in Table \ref{tab:returns}: America on the top left, Europe in the middle, and East Asia and Oceania in the bottom right. Note that the colour grading depends on the scale, but in all cases the closer to dark blue the stronger the dependence, and the closer to dark red the weaker the dependence.

Regarding TailCoR, all estimates are well above one -- the minimum is 1.37 -- and with small standard deviations (between 0.04 and 0.13) reflecting the fact that markets are dependent and with heavy tails. Expectedly, for every market the diagonal elements are the highest. These elements measure TailCoR of one market with itself, which can be interpreted as a measure of tail risk. The average TailCoR of an index with the rest of world varies from 1.57 for Bovespa to 1.87 for AEX. 

More interestingly, the heat map shows clearly a geographical clustering. The most dependent markets are in North America (S\&P500 and NASDAQ and Toronto Stock Exchange), all in dark blue and with TailCoRs above 2.1. By contrast, the remaining American markets have TailCoR of about 1.7 (interestingly enough, South American markets are less related between them than with North American markets). The next block is Europe that is mostly in the green \& dark green range (TailCoR is in the range 1.8 -- 2.2). Among these markets, the most related is AEX -- Netherlands is a very open economy and a European cross road -- and the less ATX -- Austria is the furthest geographically. The third block is Asia and Oceania with relatively low TailCoRs. The most dependent market is KOSPI -- South Korea is another small open economy and very export oriented. 
 
TailCoR within blocks is weaker than between blocks, especially between Asia and Oceania with the rest of the world. However, the European and the North American blocks are fairly related with TailCoR around 1.9 or higher.

The heat map for the linear component reveals that the source of the geographical cluster is linear. All linear components are above one, with a minimum of 1.03 and a maximum of 1.39 (diagonal elements excluded that by definition equal 1.41), and all standard deviations are very small. Within the blocks, and on average, the European block shows the higher linear dependence (1.22), followed by North America (1.18), South America (1.15), and Asia and Oceania (1.13).

The heat map for the nonlinear component shows a different pattern. All nonlinear components are above one and standard deviations are small (though not as small as for the linear component, which is expected since this component captures the dependence on the tails of the distribution). North American markets have the highest nonlinear relations, not only between them but also with the rest of the world. Some Asian indexes also show high nonlinear components, even higher than for European indexes, like KOSPI, SSEC, and STRTIM. The main diagonal measures the thickness of the tails for each market and, in fact, the correlation of the main diagonal with the kurtosis in Table \ref{tab:returns} is 99.8\%.


\begin{figure}
  \caption{Full sample results -- comparing measures}\label{fig:competing}
  \begin{center}
    \subfloat[$\theta^-(<0.025)$]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{Downside}} 
    \subfloat[$\theta^+(>0.975)$]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{Upside}} \\
    \subfloat[$\tau_p$]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{copula}}
    \subfloat[$\tau_{np}$]{\includegraphics[angle=0,height =6cm,width=.40\linewidth]{nonparam}} \\
\begin{tabular}{p{13cm}}
%\scriptsize Heat maps for comparing measures. The colour grading depends on the scale\\ 
\end{tabular}
  \end{center}
\end{figure}

Turning to the comparing measures, $\tau_p$ and $\tau_{np}$ show the same geographical clustering as TailCoR, though the contrast between and within regional blocks is sharper, in particular for $\tau_p$. This clustering is also visible in the heat map for $\theta^-(<0.025)$, though more blurred, and less visible for $\theta^+(>0.975)$. Table \ref{tab:correlations} displays the matrix of sample correlations between $\mbox{TailCoR}^{0.975} $, $\theta^+(>0.975)$, $\theta^-(<0.025)$, $\tau_p$, and $\tau_{np}$. The sample correlations are computed by vectorizing the upper triangle of the matrices of estimates (hence without the diagonal elements that are 1 by definition, and would artificially inflate the correlations), and calculating the Pearson correlations between them. The correlations of TailCoR with the other measures vary between 0.39 and 0.89. TailCoR highly correlates with $\tau_p$ and $\tau_{np}$, mildly correlates with $\theta^-(<0.025)$, and weakly correlates with $\theta^+(>0.975)$ (as a matter of consistency, one can see that $\tau_{np}$ and $\tau_p$ strongly or mildly correlate with all other measures). Overall, we conclude that for large samples TailCoR provides empirical results that are in line with equivalent measures.



\begin{table}
\begin{center}
%\scriptsize
\caption{Empirical correlations between all measures} \label{tab:correlations}
\begin{tabular}{cccccccc}
 \hline\hline
					& $\text{TailCoR}^{0.975}$& $\theta^{-}(<0.025)$	& $\theta^{+}(>0.975)$	& $\tau_p$& $\tau_{np}$  \\ 
$\text{TailCoR}^{0.975}$	& 1.00 				& 0.51				& 0.39				& 0.84	& 0.80 		\\ 
$\theta^{-}(<0.025)$		& 0.51				& 1.00				& 0.59				& 0.69	& 0.70 		\\ 
$\theta^{+}(>0.975)$		& 0.39				& 0.59				& 1.00				& 0.57	& 0.61 		\\ 
$\tau_p$				& 0.84				& 0.69				& 0.57				& 1.00	& 0.96 		\\ 
$\tau_{np}$			& 0.80				& 0.70				& 0.61				& 0.96	& 1.00 		\\ 
\hline \hline
\multicolumn{6}{p{12cm}}{\footnotesize{Empirical correlations between $\mbox{TailCoR}^{0.975} $, $\theta^+(>0.975)$, $\theta^-(<0.025)$, $\tau_p$, and $\tau_{np}$. The correlations are computed by vectorizing the upper triangle of the matrices of estimates, and calculating the Pearson correlations between them.}}
\end{tabular}
\end{center}
\end{table}
 

Next, we move to the rolling window exercise. Panels (a), (b) and (c) of Figure \ref{fig:mess} display the dynamic evolution of TailCoR, $\tau_p$, and $\tau_{np}$ respectively and for all pairs of market indexes.\footnote{Alternatively to rolling a window, one could think of a dynamic conditional TailCoR. The dynamic conditional extension would be in spirit similar to \cite{LeeLong}. This is left for future research, as explained in the conclusions.} The exceedance correlations could not be computed due to lack of extreme observations. All TailCoRs are always larger than one, and they show a pattern in line with the financial and economic events that happened during the sample period -- as explained in detail below. The tail dependence coefficients also show a recognisable pattern, though there is a larger variability across coefficients, both cross-sectionally and across time. That is, we do not observe increased clustering in times of crisis.

\begin{figure}
\caption{TailCoR and tail dependence coefficients}
\begin{center}
\subfloat[TailCoR]{\includegraphics[angle=0,width=0.45\linewidth]{TCAllPairs.eps}} \hspace{0.15cm}
\subfloat[$\tau_{np}$]{\includegraphics[angle=0,width=0.45\linewidth]{NonParametricAllPairs.eps}}\\
\subfloat[$\tau_p$]{\includegraphics[angle=0,width=0.45\linewidth]{StudentTAllPairs.eps}}
\end{center}
{\footnotesize \vspace{-0.35cm} Panel (a) shows the evolution of TailCoR for all pairs of market indexes, while panels (b) and (c) show the non-parametric and parametric tail dependence coefficients.}
\label{fig:mess}
\end{figure}


Figure \ref{fig:dynamic} focuses on TailCoR (panel a) and its nonlinear (panel b) and linear components (panel c). For the sake of visibility and interpretation, each line is the cross-sectional average of one index with respect to the others. For instance, the value of TailCoR for S\&P500 in 2000--2002 is the average TailCoR of S\&P500 with respect to all the other indexes on that period.

\begin{figure}
\caption{TailCoR and its components}
\begin{center}
\subfloat[TailCoR]{\includegraphics[angle=0,width=0.45\linewidth]{TCCrossSecAverage.eps}} \hspace{0.15cm}
\subfloat[Nonlinear component]{\includegraphics[angle=0,width=0.45\linewidth]{NonLinearCrossSecAverage.eps}} \\
\subfloat[Linear component]{\includegraphics[angle=0,width=0.45\linewidth]{LinearCrossSecAverage.eps}}
\end{center}
{\footnotesize \vspace{-0.35cm} Panel (a) shows the evolution of TailCoR for all market indexes. Each line is the cross-sectional average of one market index with respect to the others. Panels (b) and (c) show the evolution of the nonlinear and linear components respectively.}
\label{fig:dynamic}
\end{figure}

We also here observe that all TailCoRs are larger than 1 for all windows. The ups and downs show a pattern that is clearly identified with financial, economic and political events. In general TailCoR increases in crises periods, when markets become more dependent. Related with this, the variability of TailCoRs across the globe decreases in crises. During 2000-2004, the range of TailCoRs is 1.2 -- 1.7. In 2005, all TailCoRs decrease, concentrating around 1.4. This a period characterised by tails nearly Gaussian. Since then, the heaviness and the tail co-movements increase steadily. March 2007 has been identified as the beginning of the financial crisis (\cite{Acharya:2009}). TailCoR decreases between 2007 and 2008, but picks up again in 2008, when further troubles in the financial industry were made public. TailCoR then lowers for the next three years, though there is a small peak around 2011-2012 due to the European sovereign debt crisis. These are years of bonanza in financial markets and the economy overall. In 2016, there were a number of corrections worldwide that are reflected in the increase of TailCoR. The last increase, to levels comparable to the 2008 Great Financial Crisis, is due to COVID-19.
%{\color{red} in this text I miss what happened in the great crisis, mainly 2009. It seems TailCoR decreased there; can this be? Should we not explain this? I find this paragraph "disappointing" for the 2009 year which is not mentioned. May the "for the next three years" meant 2010-2012? If so, great, but then we should say it. Right now we say it increases in 2008 and then decreases the next three years, which logically includes 2009.}

Panels (b) and (c) reveal that the pattern of TailCoR is driven by the nonlinear component. The linear component evolves  smoothly while the nonlinear component is more volatile and reacts faster to the events that drive financial markets. COVID-19 is a case in point. Though the linear component has increased by 0.05 for every index, the nonlinear component increases significantly more.








==> RV_Conclusions_JoE.tex <==
\section{Conclusions}
We have introduced TailCoR, a metric for tail correlations that is a function of linear and nonlinear components, the latter characterised by the heaviness of the tails. TailCoR is exact for any probability level, it does not depend on any specific distributional assumption, and no optimisations are needed. Monte Carlo simulations reveal its goodness in finite samples. An empirical illustration to a panel of 21 market indexes around the world shows an increase of TailCoR during the financial crisis that was due to a surge of linear and nonlinear components, while the surge during the COVID-19 crisis was mostly due to the nonlinear component.

Several extensions are possible. One is conditional TailCoR, which would be based on the conditional IQR of the projection ($\mbox{IQR}^{(j\,k)\,\xi}_t = \mbox{Q}^{(j\,k)\,1-\xi}_t-\mbox{Q}^{(j\,k)\,\xi}_t$), where the time varying quantiles are regressed on the financial and economic determinants of tail correlations.
%{\color{red}I do not get this at all}
%are specified similarly to above:
%\begin{eqnarray*}
%\mbox{Q}^{(j\,k)\,\xi}_t &=& \omega^{\xi} + \bm{\beta}^{\xi} \mathbf{W}_{t-1} \mbox{ and }\\
%\mbox{Q}^{(j\,k)\,1-\xi}_t &=& \omega^{1-\xi} + \bm{\beta}^{1-\xi} \mathbf{W}_{t-1},
%\end{eqnarray*}
%where $\mathbf{W}_{t-1}$ is a set of regressors.
Under ellipticity
%we disentangle the dynamic contribution of the linear and non-linear correlations
the dynamic linear correlation $\rho_{i\,j,t}$ can be estimated with a robustified version of the DCC model (\cite{BoudtDanielssonLaurent11}).
%The dynamic non-linear correlation can be computed similarly to the static case:
%\begin{equation*}
%$s(\xi,\tau,\alpha)_t = \mbox{IQR}^{(j\,k)\,\xi}_t / \sqrt{1+\rho_{j\,k,t}}$.
%\end{equation*}
%The limiting distribution of $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{\hat{Z}\,T}$ is more involving than in the static case as it is based on the asymptotic distributions for the intercept and slopes parameters of the quantile regressions, which are known since \cite{KoenkerBassett78}. Similar arguments to those of previous section follow nevertheless.

A second extension is assuming a meta-elliptical copula (\cite{KKP08} and \cite{Krajina12}), which allows for different tail indexes for the marginal distributions and the copula. In this case, the first step should be done with a monotonically increasing transformation that standardises not only for the location and scale but also for the marginal heaviness of the tails.

%A stylized fact of financial returns is volatility clustering, and hence the standardization \eqref{eq:stand} would be more accurate if $X_{j\,t}$ is subtracted and divided by the appropriate amounts at time $t$. In a sense, this has been done in the empirical application in exploiting the daily information in every window of 6 months. An alternative is to use past information. A quantile-based measure for volatility is the dynamic IQR, or $\mbox{IQR}_{j\,t}^{\tau}=\mbox{Q}_{j\,t}^{\tau}-\mbox{Q}_{j\,t}^{1-\tau}$.
%%\footnote{We can also consider the dynamic median $\mbox{Q}^{0.50}_{j\,t}$. However, another stylized fact of financial returns is its unpredictability.}
%By means of quantile regressions, \cite{CoroneoVeredas12} show that past absolute values of returns 
%%the quantile regressions
%%\begin{eqnarray*}
%%\mbox{Q}_{j\,t}^{\tau} &=& \omega^{\tau} + \beta^{\tau}|X_{j\,t-1}| \mbox{ and } \\
%%\mbox{Q}_{j\,t}^{1-\tau} &=& \omega^{1-\tau} + \beta^{1-\tau}|X_{j\,t-1}|
%%\end{eqnarray*}
%provide an $\mbox{IQR}_{j\,t}^{\tau}$ that is an accurate estimator of the volatility.
%% for $X_{j\,t}$. Similarly for $X_{k\,t}$.\footnote{Another possibility is to use a quantile regression similar to the CAViaR of \cite{EngleManganelli04}, but it is computational more complex.}



==> RV_Extensions_JoE.tex <==
%\section{Two extensions}
%In this section we show two extensions. The first is downside- and upside-TailCoR under asymmetry. The second is one TailCoR that summarizes the linear and nonlinear correlations for the entire random vector.
%ii) Negative correlation: TailCoR as explained in the previous paragraph, is designed for positive relation as it projects the pairs of observations in the 45-degree line. A simple transformation makes it suitable for negative relation.
%: though ellipticity is a very general assumption, in some cases observations show asymmetric probability contours. To cope with this possibility we show how to do the disentangling of TailCoR in the linear and nonlinear contributions under the normal mean-variance mixture.
%and iv) dynamic TailCoR.
%: it is easy to extend the vanilla definition to the dynamic case. Since a stylized fact of financial data is volatility clustering, allowing for dynamic volatility provides dynamic TailCoR.

\section{Downside and upside TailCoR under asymmetry}

It is often the case that the interest lies in a particular region of the distribution. For instance, in risk management the region of interest is where $Y_{j\,t}$ and $Y_{k\,t}$ are negative. This translates into the negative side of the distribution of $Z^{(j\,k)}_{t}$, which leads to the following definition.

\begin{description}
\item[{\bf Definition 3}] Under {\bf G1} -- {\bf G2} we define downside- and upside-TailCoR as follows:
\begin{eqnarray*}
\mbox{TailCoR}^{(j\,k)\,\xi\,-} &:=& s_0(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi\,-} \mbox{ and} \\
\mbox{TailCoR}^{(j\,k)\,\xi\,+} &:=& s_0(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi\,+},
\end{eqnarray*}
where $\mbox{IQR}^{(j\,k)\,\xi\,-} =  \mbox{Q}^{(j\,k)\,0.50} - \mbox{Q}^{(j\,k)\,1-\xi}$ is the difference between the median and the lower tail quantile, and $\mbox{IQR}^{(j\,k)\,\xi\,+} = \mbox{Q}^{(j\,k)\,\xi} - \mbox{Q}^{(j\,k)\,0.50}$ is the difference between the upper tail quantile and the median.
\end{description}
%The normalization is now $2s_0(\xi,\tau)$. It makes $\mbox{TailCoR}^{(j\,k)\,\xi\,-}$ and $\mbox{TailCoR}^{(j\,k)\,\xi\,+}$ comparable with the full--fledged TailCoR.
%\footnote{The normalization $s_g^*(\xi,\tau)$ is the inverse of $\mbox{IQR}^{(j\,k)\,\xi\,-}$ under Gaussianity and uncorrelation, in the same way as $s_g(\xi,\tau)$ is the inverse of $\mbox{IQR}^{(j\,k)\,\xi}$ under the same conditions. By noting that the Gaussian distribution is elliptical, and by adding and subtracting the median, we obtain the relation between the two normalizations: $\mbox{IQR}^{(j\,k)\,\xi} =  (\mbox{Q}^{(j\,k)\,\xi} - \mbox{Q}^{(j\,k)\,0.50}) + (\mbox{Q}^{(j\,k)\,0.50} - \mbox{Q}^{(j\,k)\,1-\xi})=2(\mbox{Q}^{(j\,k)\,0.50} - \mbox{Q}^{(j\,k)\,1-\xi})=2\mbox{IQR}^{(j\,k)\,\xi\,-}$, or $\mbox{IQR}^{(j\,k)\,\xi\,-}=\mbox{IQR}^{(j\,k)\,\xi}/2$. Hence $s_g^*(\xi,\tau)=2/\mbox{IQR}^{(j\,k)\,\xi}=2s_g(\xi,\tau)$.}
%The upside TailCoR is defined similarly
%\begin{equation}\label{eq:upside}
%\mbox{TailCoR}^{(j\,k)\,\xi\,+} := 2s_g(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi\,+},
%\end{equation}
%where $\mbox{IQR}^{(j\,k)\,\xi\,+} = \mbox{Q}^{(j\,k)\,\xi} - \mbox{Q}^{(j\,k)\,0.50}$, i.e. the difference between the upper tail quantile and the median. 
%Under ellipticity, the projection $Z^{(j\,k)}_{t}$ is symmetric and downside and upside TailCoRs are equal to the full-fledged TailCoR.
The value added of downside and upside TailCoRs is therefore put forward under asymmetry. We model asymmetry 
%Due to the symmetry of the elliptical distribution, the downside and upside TailCoRs under {\bf E1}-{\bf E5} are the same.
%\begin{equation*}
%\mbox{TailCoR}^{(j\,k)\,\xi\,D} = \mbox{TailCoR}^{(j\,k)\,\xi\,U} = s_g^*(\xi,\tau)\frac{1}{2}s(\xi,\tau,\alpha)\sqrt {1+\rho_{j\,k}},
%\end{equation*}
%However, under asymmetry the downside and upside are different, as shown in detail in the third extension.
%\subsection{TailCoR under asymmetry}
%Though ellipticity is a fairly general assumption, in some cases observations may show asymmetric probability contours, which can be modeled
with a normal mean-variance mixture (or NMVM, see e.g. \cite{MenciaSentana09} and \cite{BLV}), i.e. $\mathbf{X}_t =_d \bm{\mu} +  \mathcal{R}_{\alpha\,t}^{2}\bm{\gamma}+ \mathcal{R}_{\alpha\,t}\bm{\Lambda}\bm{\Upsilon}_t$,
%{\color{red} this does not seem to be exactly the type of mixture we described in our paper, while it should. What do I miss? Also, should we not make that link, since we mention our paper plus the Forbes-Wraith paper in the Introduction. It would be more consistent}
 where $\bm{\Upsilon}_t$ is a standardized multivariate Gaussian distribution, and $\bm{\gamma}$ is a vector of parameters that capture the asymmetry.
%In the case of the LSMN $\mathbf{X}_t =_d \bm{\mu} +  \mathcal{R}_{\alpha\,t}\bm{\Lambda}\bm{\Lambda}'\bm{\gamma}+ \mathcal{R}_{\alpha\,t}^{1/2}\bm{\Lambda}\mathbf{W}_t$.
The most prominent distribution that belongs to this family is the generalized hyperbolic, as it nests the hyperbolic, normal gamma, and normal inverse Gaussian, among others. As the elliptical family, the NMVM family enjoys the property of affine invariance, i.e. it is closed under linear operations, which means that the projection $Z^{(j\,k)}_t$ is also a NMVM random variable. 

%The relation between the IQR and the dispersion parameter is now $\mbox{IQR}^{\tau}_j = k(\tau,\alpha,\gamma_j)\sigma_{X_j}$ where $\gamma_j$ is the asymmetry parameter of the $j$th random variable.
The vector of unknown parameters is now $\bm{\theta}=(\bm \mu, \bm \Sigma, \bm \gamma,\alpha)$. While assumptions {\bf E1} and {\bf E2} have to be trivially modified, {\bf E3} -- {\bf E5} remain unchanged. We re-name them as {\bf A1} -- {\bf A5}. In order to disentangle the linear and nonlinear correlations, uniform asymmetry is needed, as stated in the following assumption.

\begin{itemize}
\item[\bf A6] $\gamma=\gamma_j=\gamma_k$, $\forall j,k=1,\ldots,N$. 
\end{itemize}

This assumption does not imply symmetry, which is a particular case when $\gamma=0$. Rather, it implies that all the random variables are equally asymmetric. Though uniform asymmetry may seem restrictive, empirical results -- see for instance \cite{Jondeau10} -- show that the estimated asymmetries do not show large discrepancies, which is also corroborated in the empirical illustration.

Under asymmetry, the relation between $X_{j\,t}$ and $X_{k\,t}$ is not the same over the domain of the observations. For instance, \cite{LoginSolnik01} and \cite{Jondeau10} find that the dependence across asset returns may be stronger in bearish than in bullish conditions. These asymmetric dependencies are captured with 
%TailCoR in the theorem above is not able to capture these differences. But a simple variation does, which leads to downside and upside TailCoR under asymmetry. The variation consists of using
semi--variances, semi--interquantile ranges, and semi--correlations. The prefix "semi" means that we use observations that are in a certain range. For instance, the positive semi--interquantile range is the difference between the upper quantile and the median, as used in the upside-TailCoR.

Let $\sigma_j^{2\,+}$ be the positive semi--variance and $\mbox{IQR}^{\tau\,+}_j = \mbox{Q}^{\tau}_j - \mbox{Q}^{0.50}_j$ be the positive semi--interquantile range of $X_{j\,t}$ of order $\tau$. The relation between both is given by $\mbox{IQR}^{\tau\,+}_j=k(\tau,\alpha,\gamma)^{+}\sigma_j^{+}$. Similarly, $\sigma_j^{2\,-}$ and $\mbox{IQR}^{\tau\,-}_j = \mbox{Q}^{0.50}_j - \mbox{Q}^{1-\tau}_j$ are the negative semi--variance and the negative semi--interquantile range, which are related by $\mbox{IQR}^{\tau\,-}_j=k(\tau,\alpha,\gamma)^{-}\sigma_j^{-}$. Similar definitions apply for $X_{k\,t}$. We also need the positive and negative semi--correlations between $X_{j\,t}$ and $X_{k\,t}$: the former is defined as $\rho^+_{j\,k}=\sigma_{j\,k}^{+}/\sigma_j^{+}\sigma_k^{+}$, where $\sigma_{j\,k}^{+}$ is the positive semi--covariance. Likewise for the negative semi--correlation.

By the affine invariance of the NMVM family, it follows that semi--interquantile ranges in Definition 3 equal $\mbox{IQR}^{(j\,k)\, \xi\,+} =k(\xi,\alpha,\gamma)^{+}\sigma_{(j\,k)}^{+}$ and $\mbox{IQR}^{(j\,k)\, \xi\,-} =k(\xi,\alpha,\gamma)^{-}\sigma_{(j\,k)}^{-}$, where $\sigma_{(j\,k)}^{2\,+}$ and $\sigma_{(j\,k)}^{2\,-}$ are the positive and negative semi--variances of the projection $Z^{(j\,k)}_t$. Further properties of the semi--moments are found in Appendix P. 

Under the NMVM family of distributions, the optimal projection may not be on the 45- or the 135-degree lines, but on a line with angle $\phi$  that maximizes the variability of the projection. The procedures explained under {\bf G1} -- {\bf G2} apply here. The following theorem shows downside- and upside-TailCoR under asymmetry.

\begin{description}
\item[{\bf Theorem 5}]
Let $X_{j\,t}$ and $X_{k\,t}$ be two elements of the random vector $\mathbf{X}_t$ that fulfill assumptions {\bf A1} -- {\bf A6}. Let $\rho^+_{j\,k}$ and $\rho^-_{j\,k}$ be the positive and negative semi--correlations, and let $s(\xi,\tau,\alpha,\gamma)^{+}$ and $s(\xi,\tau,\alpha,\gamma)^{-}$ be two continuous and monotonically decreasing functions of $\alpha$. Then
\begin{eqnarray*}
\mbox{TailCoR}^{(j\,k)\,\xi \,-} &=&2s_g(\xi,\tau)s(\xi,\tau,\alpha,\gamma)^{-}\sqrt{1+  2 |\rho^-_{j\,k}| |\sin \phi \cos \phi|} \quad \mbox{and} \\
\mbox{TailCoR}^{(j\,k)\,\xi \,+} &=&2s_g(\xi,\tau)s(\xi,\tau,\alpha,\gamma)^{+}\sqrt{1+ 2 |\rho^+_{j\,k}| |\sin \phi \cos \phi|},
\end{eqnarray*}
where $s_g(\xi,\tau)$ is a normalization such that, under independence, we have $\mbox{TailCoR}^{(j\,k)\,\xi \,-}=\mbox{TailCoR}^{(j\,k)\,\xi \,+}=1$, the reference value.
\end{description}

\begin{description}
\item[{\bf Proof}] See Appendix P.
\end{description}

The normalization is now $2s_g(\xi,\tau)$. It makes $\mbox{TailCoR}^{(j\,k)\,\xi\,-}$ and $\mbox{TailCoR}^{(j\,k)\,\xi\,+}$ comparable with the full--fledged TailCoR. When $\phi$ equals $\frac{\pi}{4}$ or $\frac{3\pi}{4}$ (i.e., projections in the 45- and 135-degree lines), $\sqrt{1+ 2 |\rho^+_{j\,k}| |\sin \phi \cos \phi|}$ equals $\sqrt{1+ |\rho^+_{j\,k}|}$. The downside- and upside-TailCoR can differ because either the linear and/or the nonlinear correlations are different. Estimation follows the same steps as in the previous estimators except for the use of semi metrics.

%Admittedly, under the NMVM family of distributions, the optimal projections may not be the 45- or the 135-degree line. The theorem above can be easily modified for projection in a generic angle $\phi$. Then 
%\begin{eqnarray*}
%\mbox{TailCoR}^{(j\,k)\,\xi \,+} &=&2s_g(\xi,\tau)s(\xi,\tau,\alpha,\gamma)^{+}\sqrt{1+ 2 \sin \phi \cos \phi |\rho^+_{j\,k}|} \quad \mbox{and} \\
%\mbox{TailCoR}^{(j\,k)\,\xi \,-} &=&2s_g(\xi,\tau)s(\xi,\tau,\alpha,\gamma)^{-}\sqrt{1+ 2 \sin \phi \cos \phi|\rho^-_{j\,k}|}.
%\end{eqnarray*}

%: semi interquantile ranges for the standardization of $X_j$ and $X_k$, and robust semi correlations.

%\david{this paragraph on inference is from the previous section of negative tailcor}The estimators follow the same lines as in previous section. The limiting distribution is similar to that of $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{\hat{Z},T}$ except that the asymptotic variance-covariance matrix needs to be adapted since the interquantile range of the projection is not symmetric.\footnote{The resulting expression is similar to that of the Corollary with $1-\xi=0.50$ for upside, and $\xi=0.50$ and $1-\xi=\xi$ for downside.}


%This allows to disentangle between the linear and nonlinear correlations, the latter depending on $\alpha$ and $\gamma$, as shown in the following theorem.

%\begin{description}
%\item[{\bf Theorem 5}] {\it Under {\bf A1}-{\bf A6}
%\begin{equation*}
%\mbox{TailCoR}^{(j\,k)\,\xi} = s_g(\xi,\tau)s(\xi,\tau,\alpha, \gamma)\sqrt{1+\rho_{j\,k}}.
%\end{equation*}
%%where $\bm\gamma_{(j\,k)}=(\gamma_j,\gamma_k)$.
%}
%\end{description}
%
%\begin{description}
%\item[{\bf Proof}] See Appendix P.
%\end{description}

%Figure \ref{fig:asymtailcor} studies the effect of the asymmetry in the nonlinear correlation for the Student-t with $\alpha=2.5$ (left plot) and ES (right plot) with $\alpha=1.5$ distributions. The asymmetry parameters $\gamma_1$ and $\gamma_2$ range from -2 to 2. The plots show
%%Mote Carlo results, available under request, show
%that the nonlinear correlation increases as the asymmetries increase in the same direction for $X_{j\,t}$ and $X_{k\,t}$, and it decreases as the asymmetries move in opposite directions.
%Visually, the former corresponds to a scatter plot with extreme pairs of observations only in either the north-east of the south-west quadrants, which creates an increase in the interquantile of the projection. The latter correspond to extreme pairs of observations in either the south-east or the north-west quadrants, which creates a concentration of projected dots towards the origin, and hence a smaller interquantile range than in the case of symmetry.
%
%\begin{center}[FIGURE \ref{fig:asymtailcor} ABOUT HERE]\end{center}

%\begin{figure}[!ht]
%  \caption{Effect of asymmetry in the nonlinear correlation}\label{fig:asymtailcor}
%  \begin{center}
%    \subfloat[Student-t]{\includegraphics[angle=0,width=.45\linewidth]{figures/smallstudentnonlineargamma12}}
%    \hspace{0.6cm}
%    \subfloat[ES]{\includegraphics[angle=0,width=.45\linewidth]{figures/smallesdnonlineargamma12}} \\
%\begin{tabular}{p{14.5cm}}
%\scriptsize Surface plots with the effect of the asymmetry in the nonlinear correlation for the bivariate Student-t with $\alpha=2.5$ (left plot) and ES (right plot) with $\alpha=1.5$ distributions. The asymmetry parameters $\gamma_1$ and $\gamma_2$ range from -2 to 2. \\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%Figure \ref{fig:tailasymtailcor} shows the effect of the tail index and asymmetry in the nonlinear correlation for the Student-t (left plot) and ES (right plot) distributions. While $\gamma_1$ is set to zero, $\gamma_2$ ranges from -2 to 2. The effect of the asymmetry increases with the tail thickness. One on extreme, when the distributions are highly heavy tailed, the nonlinear correlation increases rapidly with $\gamma_2$. On the other extreme, as the distribution approaches to the Gaussian, i.e. as $\alpha$ approaches to $\infty$ and $2$ for the Student-t and ES respectively, $\gamma_2$ looses meaning. This is because $\mathcal{R}_{\alpha\,t}$ becomes a degenerate random variable and the term $\mathcal{R}_{\alpha\,t}^{2}\bm{\gamma}$ is not random and hence it becomes a location shift.
% 
%\begin{figure}[!ht]
%  \caption{Effect of tails and asymmetry in the nonlinear correlation}\label{fig:tailasymtailcor}
%  \begin{center}
%    \subfloat[Student-t]{\includegraphics[angle=0,width=.45\linewidth]{figures/smallstudentnonlinearalphagamma}}
%    \hspace{0.6cm}
%    \subfloat[ES]{\includegraphics[angle=0,width=.45\linewidth]{figures/smallesdnonlinearalphagamma}} \\
%\begin{tabular}{p{14.5cm}}
%\scriptsize Surface plots with the effect of the tails and asymmetry in the nonlinear correlation for the bivariate Student-t (left plot) and ES (right plot) distributions. $\gamma_1$ is set to zero and $\gamma_2$ ranges from -2 to 2. \\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%The implementation under asymmetry is the same as under ellipticity, and the asymptotic distribution of the estimators follows from the corollary of Theorem 2. This is because $\mbox{TailCoR}^{(j\,k)\,\xi}$ uses all the observations in equal manner, regardless of the part of the region of the distribution they lay in.

%Under asymmetry the correlations (linear and nonlinear) are not the same over the domain of the observations. For instance, \cite{LoginSolnik01} and \cite{Jondeau10} find that the dependence across asset returns may be stronger in bearish than in bullish conditions. TailCoR in the theorem above is not able to capture these differences. But a simple variation does, which leads to downside and upside TailCoR under asymmetry.
%
%The variation consists of using semi variances, semi interquantile ranges, and semi correlations. The term semi relates to the use of observations that are in a certain range. For instance, the positive semi interquantile range is the difference between the upper quantile and the median, as used in the upside TailCoR under {\bf G1}-{\bf G2}.



%As mentioned below, a simple test for asymmetry can be constructed based on these estimators.


%\subsection{Negative correlation}
%
%$\mbox{TailCoR}^{(j\,k)\,\xi}$, as defined so far, is designed for positive relations as it projects the pairs of observations onto the 45-degree line. Left plot of Figure \ref{fig:negtailcor} shows the projection on that line when the relation is negative: it leads to $Z^{(j\,k)}$ very concentrated around the origin and TailCoR smaller than that leads to the false conclusion that tails are thinner than Gaussian. A simple transformation makes $\mbox{TailCoR}^{(j\,k)\,\xi}$ suitable for negative relations: instead of projecting onto the 45-degree line, we project onto the 135-degree line, as depicted in the right plot of Figure \ref{fig:negtailcor}. Following similar trigonometric arguments as before, the projection is
%\begin{equation*}
%Z^{(j\,k)}_{t} = \frac{1}{\sqrt{2}}(Y_{j\,t} - Y_{k\,t}).
%\end{equation*}
%Under {\bf G1}-{\bf G2}, the definition remains, i.e. $\mbox{TailCoR}^{(j\,k)\,\xi} := s_g(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi}$. However, under {\bf E1}-{\bf E5}, the expression is slightly modified:
%\begin{equation*}
%\mbox{TailCoR}^{(j\,k)\,\xi} = s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt {1-\rho_{j\,k}}.
%\end{equation*}
%The asymptotic distributions of the Theorem and the Corollary above are not modified. Projecting onto the 45- or 135-degree line is a user choice. Visual inspection of the scatter plots for choosing the projection is only feasible when $\mathbf{X}_t$ is small dimensional. For vast dimensions we propose the following automatized method. Let $Z^{(j\,k)}_{45\,t}$ and $Z^{(j\,k)}_{135\,t}$ be the projections onto the 45- and 135-degree lines for the pair $(j\,k)$, and let $\mbox{IQR}^{(j\,k)\,\xi}_{45}$ and $\mbox{IQR}^{(j\,k)\,\xi}_{135}$ be the corresponding IQRs. If $\mbox{IQR}^{(j\,k)\,\xi}_{45}>\mbox{IQR}^{(j\,k)\,\xi}_{135}$  then use $Z^{(j\,k)}_{45\,t}$, otherwise use $Z^{(j\,k)}_{135\,t}$. If $\mbox{IQR}^{(j\,k)\,\xi}_{45}=\mbox{IQR}^{(j\,k)\,\xi}_{135}$ there is neither linear nor nonlinear correlation and $\mbox{TailCoR}^{(j\,k)\,\xi}$ computed in either way gives the same result.
%
%\begin{center}[FIGURE \ref{fig:negtailcor} ABOUT HERE]\end{center}

%\begin{figure}[!ht]
%  \caption{A diagrammatic representation of TailCoR for negative relation}
%  \begin{center} \vspace{0.2cm}
%%    \subfloat[$T=500$]{
%    \includegraphics[angle=0,width=.45\linewidth]{figures/Diagram2} \hspace{0.5cm}
%%    \vspace{-0.5cm}
%%    \subfloat[$T=500$]{
%    \includegraphics[angle=0,width=.45\linewidth]{figures/Diagram3}
%%    } \\ \vspace{-0.5cm}
%  \end{center}
%     {\footnotesize  \vspace{0cm} Scatter plots, along with the 45- (left) and 315-degree (right) lines, where  $X_j$ and $X_k$ are negatively related (the pairs are depicted with circles). Projecting the observations onto the 45- or 315-degree lines produces the random variable $Z^{(j\,k)}$, depicted with squares.}
%  \label{fig:negtailcor}
%\end{figure}

%\begin{figure}[!ht]
%  \caption{A diagrammatic representation of TailCoR for negative relation}\label{fig:negtailcor}
%  \begin{center}
%    \subfloat[Projection in the 45-degree line]{\includegraphics[angle=0,width=.45\linewidth]{figures/Diagram2}}
%    \hspace{0.6cm}
%    \subfloat[Projection in the 135-degree line]{\includegraphics[angle=0,width=.45\linewidth]{figures/Diagram3}} \\
%\begin{tabular}{p{14.5cm}}
%\scriptsize Scatter plots, along with the 45- (left) and 135-degree (right) lines, where  $X_j$ and $X_k$ are negatively related (the pairs are depicted with circles). Projecting the observations onto the 45- or 135-degree lines produces the random variable $Z^{(j\,k)}$, depicted with squares. \\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%\subsection{One TailCoR for the random vector}
%
%\david{perhaps three extensions. The two, multivariate and one TailCoR, under ellipticity. The second relaxing ellipticity.}
%
%It may be of interest to have a unique tail correlation for the random vector $\mathbf{X}_t$, instead of pairwise measures. Following similar trigonometric arguments to the bivariate case, it can be shown that the projection is \david{is this the projection under ellipticity? optimality? projection under a generic angle.}
%\begin{equation*}
%Z_t^0 = \sum_{i=1}^{N} \frac{Y_{i\,t}}{\sqrt{N}}.
%\end{equation*}
%%This is done by first projecting a pair onto the corresponding \textit{marginal} 45-degree line. Then this projection and a third element of the random vector is projected onto another \textit{marginal} 45-degree line. And this process continues until the last element. The final projection is
%%\begin{equation*}
%%Z_t = \sum_{i=1}^{N-2} \frac{1}{2^{i/2}}Y_{i\,t} + \frac{1}{2^{N-1/2}}(Y_{N-1\,t} + Y_{N\,t})
%%\end{equation*}
%%when all the \textit{marginal} projections are on the 45-degree line.
%Let $\mbox{IQR}^{0\,\xi}$ be the tail interquantile range of $Z_t^0$, which leads to the new definition of TailCoR.
%\begin{description}
%\item[{\bf Definition 4}] Under {\bf G1}-{\bf G2}, TailCoR between $(X_{1\,t},\cdots,X_{N\,t})$ is
%\begin{equation*}
%\mbox{TailCoR}^{0\,\xi}  := s_g(\xi,\tau)\mbox{IQR}^{0\,\xi}.
%\end{equation*}
%\end{description}
%Under the elliptical assumptions we disentangle $\mbox{TailCoR}^{0\,\xi}$ as shown in the following theorem.
%\begin{description}
%\item[{\bf Theorem 5}] Under {\bf E1}-{\bf E5}, TailCoR of $(X_{1\,t},\cdots,X_{N\,t})$ is
%\begin{equation} \label{eq:one}
%\mbox{TailCoR}^{0\,\xi}  = s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt{1+\frac{2}{N}\sum_{j=1,k=2,j > k}^{N}|\rho_{j\,k}|}.
%\end{equation}
%\end{description}
%
%\begin{description}
%%\item[{\bf Proof}] It follows the same lines as the proof of Theorem 1.
%\item[{\bf Proof}] See Appendix P. \david{change because of the absolute value of rho}
%\end{description}
%
%As in the pairwise case, the reference point is 1. Note that for $N=2$ we are back to Theorem 1. Also, similarly to the univariate case, \eqref{eq:one} can be transformed for being bounded between -1 and 1, and centered around 0:
%\begin{equation}\label{eq:alternativeone}
%\mbox{TailCoR}^{0\,\xi}_{alt} = \mbox{sign}(\rho)\frac{\mbox{TailCoR}^{0\,\xi} - 1}{s_g(\xi, \tau)s(\xi, \tau,\alpha)\sqrt{2} - 1},
%\end{equation}
%where $\rho=\sum_{j=1,k=2,j > k}^{N}|\rho_{j\,k}|$.
%
%This result is for the case where all the relations are positive. It can be easily extended to the case of having both positive and negative relations.
%, i.e. the value of TailCoR in the case of uncorrelation and Gaussianity.
%Under this distribution the upper bound is $\sqrt{N}$, obtained by setting all the Pearson correlation coefficients to one. The lower bound is not straightforward since positive and negative relations have to be taken into account.
%Last, under another elliptical distribution than Gaussian, even if $X_j$ and $X_k$ are linearly uncorrelated, $\mbox{TailCoR}^{\xi}$ is larger than one as $s_g(\xi,\tau)s(\xi,\tau,\alpha)>1$, as in the pairwise case.
%
%Estimation follows the same steps as for $\mbox{TailCoR}^{(j\,k)\,\xi}$ under {\bf G1}-{\bf G2}. Under the elliptical assumptions, the multivariate extension of the robust correlation estimator can be used. The asymptotic distributions under {\bf G1}-{\bf G2} and {\bf E1}-{\bf E5} are the same to those of Theorem 2 and its corollary -- since they are based on the IQR of the projection.
% --, up to a slight modification of $\omega$ to account for $N$ standardizations.




%A similarity with the downside and upside TailCoR is the normalization $2s_g(\xi,\tau)$, which is the same since the benchmark is always the Gaussian and uncorrelated process. An important difference however is that $\mbox{TailCoR}^{(j\,k)\,\xi \,+}$ and $\mbox{TailCoR}^{(j\,k)\,\xi \,-}$ are obtained by considering the downside and upside regions as independent, which leads to different linear 
%
%This relates to the downside- \& upside-TailCoR is a way that is explained below.
%
%under {\bf G1-G2} but it differs under {\bf A1}-{\bf A5} (assumption {\bf A6} is not needed anymore) as shown in the sequel.
%
%
%RELATION WITH UPSIDE AND DOWNSIDE TAILCOR
%
%Estimation procedure, estimating the correlations

%\subsection{Dynamic TailCoR}
%
%Up to now TailCoR is an unconditional measure. It is however possible to extend it to the dynamic case. A stylized fact of financial returns is volatility clustering, and hence the standardization \eqref{eq:stand} would be more accurate if $X_{j\,t}$ is subtracted and divided by the appropriate amounts at time $t$. A quantile-based measure for volatility is the dynamic IQR, or $\mbox{IQR}_{j\,t}^{\tau}=\mbox{Q}_{j\,t}^{\tau}-\mbox{Q}_{j\,t}^{1-\tau}$.\footnote{We can also consider the dynamic median $\mbox{Q}^{0.50}_{j\,t}$. However, another stylized fact of financial returns is its unpredictability.} \cite{CoroneoVeredas12} show that the quantile regressions
%\begin{eqnarray*}
%\mbox{Q}_{j\,t}^{\tau} &=& \omega^{\tau} + \beta^{\tau}|X_{j\,t-1}| \mbox{ and } \\
%\mbox{Q}_{j\,t}^{1-\tau} &=& \omega^{1-\tau} + \beta^{1-\tau}|X_{j\,t-1}|
%\end{eqnarray*}
%provide an $\mbox{IQR}_{j\,t}^{\tau}$ that is an accurate estimator of the marginal volatility for $X_{j\,t}$. Similarly for $X_{k\,t}$.\footnote{Another possibility is to use a quantile regression similar to the CAViaR of \cite{EngleManganelli04}, but it is computational more complex.} The IQR of the projection may also be time varying 
%$\mbox{IQR}^{(j\,k)\,\xi}_t = \mbox{Q}^{(j\,k)\,1-\xi}_t-\mbox{Q}^{(j\,k)\,\xi}_t$,
%where the quantile regressions depend on a set of regressors.
%%are specified similarly to above:
%%\begin{eqnarray*}
%%\mbox{Q}^{(j\,k)\,\xi}_t &=& \omega^{\xi} + \bm{\beta}^{\xi} \mathbf{W}_{t-1} \mbox{ and }\\
%%\mbox{Q}^{(j\,k)\,1-\xi}_t &=& \omega^{1-\xi} + \bm{\beta}^{1-\xi} \mathbf{W}_{t-1},
%%\end{eqnarray*}
%%where $\mathbf{W}_{t-1}$ is a set of regressors.
%Similarly to the static case, under {\bf E1}-{\bf E5} we disentangle the dynamic contribution of the linear and nonlinear correlations. The dynamic linear correlation $\rho_{i\,j,t}$ can be estimated with a robustified version of the DCC model of \cite{Engle02} (\cite{BoudtDanielssonLaurent11}). The dynamic nonlinear correlation is computed similarly to the static case:
%\begin{equation*}
%s(\xi,\tau,\alpha)_t = \frac{\mbox{IQR}^{(j\,k)\,\xi}_t}{\sqrt{1+\rho_{j\,k,t}}}.
%\end{equation*}
%The limiting distribution of $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{\hat{Z}\,T}$ is more involving than in the static case as it is based on the asymptotic distributions for the intercept and slopes parameters of the quantile regressions, which are known since \cite{KoenkerBassett78}. Similar arguments to those of previous section follow nevertheless.

%\subsection{Multivariate}
%
%So far we have only considered the pair $(j\,k)$ of random variables while the random vector $\mathbf{X}_t$ is of dimension $N$. Considering all the pairs, it leads to a $N(N+1)/2$ vector of TailCoR (including TailCoR of a random variable with itself). For the ease of exposition let $\tilde{N}=N(N+1)/2$. We denote by $\xi_{(j\,k)}$ the probability level at which we compute the IQR for the $(j\,k)$ projection. If $\xi_{(j\,k)}=\xi$ $\forall j,k$, we define the vector of TailCoR as
%\begin{equation}\label{eq:vectortailcor}
%\mbox{\bf TailCoR}^{\xi} := s_g(\xi,\tau)\mbox{\bf IQR}^{\xi},
%\end{equation}
%where $\mbox{\bf IQR}^{\xi}$ is a matrix of IQRs of the $\tilde{N} \times 1$ projections. The assumption $\xi_{(j\,k)}=\xi$ $\forall j,k$ is a simplification and it allows to have the above definition. It is nonetheless possible to relax it at the cost of notation. Under ellipticity, (\ref{eq:vectortailcor}) becomes
%\begin{equation}\label{eq:vectortailcorellip}
%\mbox{\bf TailCoR}^{\xi} = \sqrt{2}s_g(\xi,\tau)s(\xi,\tau,\alpha)\mbox{\bf R},
%\end{equation}
%where the matrix $\mbox{\bf R}$ has $(j\,k)$ element $\sqrt{\frac{1+\rho_{j\,k}}{2}}$. I.e. it is symmetric, with unitary diagonal, and off-diagonal elements bounded above and bellow by 1 and 0 respectively. This matrix has the following properties: i) similarly to the univariate case, it is invariant to location-scale shifts of $\bm{X}_t$, ii) it is semi-definite positive, iii) the minimum eigenvalue is 0 and the maximum is bounded by $N$, as their sum equals $N$ (the trace of $\mbox{\bf R}$).
%
%Estimation follows the same steps as in the univariate case under {\bf G1}-{\bf G2}:
%\begin{equation*}
%\hat{\mbox{\bf TailCoR}}^{\xi}_{\hat{\mathbf{Z}}\,T} = s_g(\xi,\tau)\hat{\mbox{\bf IQR}}^{\xi}.
%\end{equation*}
%Under the ellipticity assumptions {\bf E1}-{\bf E5}, an extra step has to be added as $s(\xi,\tau,\alpha)$ is the same for all. Let $\hat{s(\xi,\tau,\alpha)}_{h \, T}=\hat{s(\xi,\tau,\alpha)}^{(j\,k) \, T}$, $h=1,\ldots,\tilde{N}$. The nonlinear correlation is estimated by pooling the pairwise estimators: 
%\begin{equation*}
%\hat{s(\xi,\tau,\alpha)}_{T} = \frac{1}{\tilde{N}}\sum_{h=1}^{\tilde{N}} \hat{s(\xi,\tau,\alpha)}_{h \,T}.
%\end{equation*}
%Estimating by averaging estimators in a cross-sectional sense has been used in the past, see e.g. \cite{ChenJachoLinton09} for efficient instrumental variable estimators, \cite{Nolan10} and \cite{DominicyOgataVeredas12} for the estimation of the tail index within the elliptical family of distributions.
%
%The asymptotic distribution incorporates now the covariances between the sample quantiles of the marginal distributions. Let $\mathbf{Z}_t=(Z^{(1\,1)}_t,\ldots,Z^{(N-1\,N)}_t)=(Z_{1\,t},\ldots,Z_{\tilde{N}\,t})$ be the vector of projections. Likewise, let $\mathbf{Q}^{\xi}=(Q_{1}^{\xi},\ldots,Q_{\tilde{N}}^{\xi})$ be the vector of quantiles and $\hat{\mathbf{Q}}^{\xi}$ the sample counterparts. Under {\bf G1}-{\bf G2}, \cite{DominicyHormannOgataVeredas12} show that $\sqrt{T}(\hat{\mathbf{Q}}^{\xi}-\mathbf{Q}^{\xi})\rightarrow \mathcal{N}(\mathbf{0},\bm\Omega)$ where
%\begin{eqnarray*}
%\bm\Omega_{j\,j} &=& \frac{\Gamma_{j\,j}(Q^{\xi}_j)}{f^2_j(F_j^{-1}(\xi))}, \\
%\Gamma_{j\,j}(Q^{\xi}_j) &=& \sum_{t=-\infty}^{\infty} E(Y_0(Q^{\xi}_j),Y_t(Q^{\xi}_j)) \mbox{ and } \\
%Y_t(Q^{\xi}_j) &=& I\{Z_{j\,t} \leq Q^{\xi}_j \} - P(Z_{j\,t} \leq Q^{\xi}_j),
%\end{eqnarray*}
%and
%\begin{eqnarray*}
%\bm\Omega_{j\,k} &=& \frac{\Gamma_{j\,k}(Q^{\xi}_j,Q^{\xi}_k)}{f_j(F_j^{-1}(\xi))f_k(F_k^{-1}(\xi))} \forall j \neq k, \\
%\Gamma_{j\,k}(Q^{\xi}_j) &=& \sum_{t=-\infty}^{\infty} E(Y_0(Q^{\xi}_j,Q^{\xi}_k),Y_t(Q^{\xi}_j,Q^{\xi}_k)) \mbox{ and }\\
%Y_t(Q^{\xi}_j,Q^{\xi}_k) &=& I\{Z_{j\,t} \leq Q^{\xi}_j,Z_{k\,t} \leq Q^{\xi}_k \} - P(Z_{j\,t} \leq Q^{\xi}, Z_{k\,t} \leq Q^{\xi}_k).
%\end{eqnarray*}
%
%Let $\hat{\mbox{\bf Q}}^{\tau} =(\hat{\mbox{Q}}^{0.50}_1,\hat{\mbox{Q}}^{\tau}_1,\ldots,\hat{\mbox{Q}}^{0.50}_N,\hat{\mbox{Q}}^{\tau}_N)$ be the vector of sample quantiles used in the standardizations of $\mathbf{X}_t$. We denote by $Cov(\hat{\mbox{\bf Q}}^{\tau})$ its variance-covariance matrix, and $\mbox{\bf Q}^{\tau}$ the population counterpart. The following Theorem shows the asymptotic distribution of the vectorized $\hat{\mbox{\bf TailCoR}}^{\xi}_{\hat{\mathbf{Z}}\,T}$.
%
%\begin{description}
%\item[{\bf Theorem 4}] {\it Under {\bf E1}-{\bf E5}
%\begin{equation*}
%\sqrt{T}\left(vech \hat{\mbox{\bf TailCoR}}^{\xi}_{\hat{\mathbf{Z}}\,T} - vech \mbox{\bf TailCoR}^{\xi}\right) \rightarrow \mathcal{N}\left(0,4s_g(\xi,\tau)^2\left(\bm\Omega+\bm\omega\right)\right),
%\end{equation*}
%where $\bm\Omega$ is defined as above and
%\begin{equation*}
%\bm\omega = \frac{\partial \mbox{\bf Q}^{\xi}(\mbox{\bf Q}^{\tau})}{\partial \mbox{\bf Q}^{\tau}}Cov(\mbox{\bf Q}^{\tau})\frac{\partial \mbox{\bf Q}^{\xi}(\mbox{\bf Q}^{\tau})}{\partial \mbox{\bf Q}^{\tau \,'}}.
%\end{equation*}
%}
%\end{description}
%
%\begin{description}
%\item[{\bf Proof}] It follows the same lines as the proof of Theorem 2.
%\end{description}
%
%Under {\bf E1}-{\bf E5} and arranging the vector into a matrix, the definition \eqref{eq:vectortailcor} can be re-written as
%\begin{equation*}
%\mbox{\bf TailCoR}^{\xi} := f(\xi,\tau,\alpha)\mathbf{R}
%\end{equation*}
%where $\mbox{\bf TailCoR}^{\xi}$ is a $N \times N$ matrix, $f(\xi,\tau,\alpha)=s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt{2}$, and $\mathbf{R}$ is a $N \times N$ symmetric matrix with diagonal and off-diagonal elements $R_{j\,j} = 1$ and $R_{j\,k} = \frac{\sqrt{1+\rho_{i\,j}}}{\sqrt{2}}$ respectively. Hence $0 \leq R_{j\,k}  \leq 1$ $\forall j,k$.
%
%{\bf PROPERTIES OF $\mathbf{R}$???}






==> RV_Introduction_JoE.tex <==
\section{Introduction}

\subsubsection*{Empirical motivation}
Two major global crises have stricken the economy and financial markets since 2000: The 2007-2008 Great Financial Crisis and the 2020 Great Lockdown due to COVID-19. These crises highlight the importance of tail -- or rare -- events that can have different natures:  corporate and Government defaults, stock market crashes, public health emergencies, or political decisions, to name a few.
%Understanding them, measuring them, and insuring against them has become of paramount importance.

When they occur, their shock wave spreads over the economic and financial systems through large co-movements. These unfrequent events  locate on the tails of the probability distributions. From a statistical point of view, joint tail events are caused by linear and/or nonlinear correlations. Indeed, correlations on the tails may happen because variables are linearly correlated (i.e., the Pearson correlations are different from zero) and/or nonlinearly correlated, in the sense that variables are dependent at the tails of their distributions only.\footnote{Other forms of nonlinearity may occur but we do not take them into account. They can however be considered within the theory of TailCoR.}
%An illustrative example is a multivariate Student-t distribution, where the dependence between the random variables is through the linear correlations and the tail index.
%of the former is a bivariate Gaussian process with correlation different from zero, while an uncorrelated Student-t bivariate process is an example of the latter.

% in a tail sense. Diagrammatically, the latter happens when the cloud of points in a scatter plot between the returns of two securities does not have a well defined direction for small and moderate values but the tail events co--move.

The analysis of tail correlations and their linear and nonlinear components has numerous financial applications. \cite{GGV15} document that while the linear dependence between short selling activity and asset returns is very weak, the correlation between extreme negative returns and extreme increases in short selling is highly significant. This finding sheds light on the contradiction between the widespread view among practitioners that short selling has mostly positive effects, and the bans of this activity by the competent authorities. \cite{PoonRockingerTawn04} argue that in the case of a portfolio the relationships among the constituents when they are on the tails give a better understanding on the tail behavior of the portfolio. The disentangling between the linear and nonlinear components allows not only to design portfolio allocation procedures that minimize the linear risk but also the tail risk of the portfolio (\cite{JKV00}).

Tail correlations also relate to the literature of tail risk spillovers using quantiles (namely VaR and CoVaR of \cite{CoVaR2016}). In this context, \cite{HautSchaSchie2015} introduce systemic risk betas as the total time-varying marginal effect of a firm's VaR on the system's VaR. These effects are computed as a function of the interdependence between firm's tail risk exposures. \cite{HardWangYu2016} propose a semiparametric measure to estimate systemic interconnectedness across financial institutions based on tail-driven spillover effects in a high dimensional network. \cite{CheSun2020} use this methodology for studying systemically important insurers.

%as shown in \cite{PoonRockingerTawn04}. For instance,
%%let two portfolios formed by securities with returns that are dependent. The investor that holds these portfolios may be exposed to linear and nonlinear sources of risk.
%a portfolio of securities that are nonlinear risk independent has thinner tails than a portfolio with securities that are nonlinear risk dependent. Therefore, the investment decision does not only depend on the investor's risk appetite, but also on her/his preferences for linear and nonlinear risks. Disentangling them allows for a more effective risk management.


%{\bf ROBUST PREFERENCES?}
%By the same token, the portfolio linear risk can be reduced (or diversified), increased (concentrated) or remained steady (neutral) with respect to the securities depending on the sign of the linear correlation.

%Several authors have proposed measures that capture co-movements on the tails. The tail dependence

\subsubsection*{Literature review}

Several statistical and econometric measures have been proposed to assess the degree of tail dependence. The tail dependence coefficients (also called extremal dependence structures and co-exceedance probabilities) stemming from extreme value theory (EVT henceforth) are the most used. These coefficients rely on two building blocks. The first is the assumption that tails of the distribution (either the joint and/or the marginal distributions) asymptotically decay according to a power law (see \cite{KiriRooWadsSeg2019} and \cite{RooSegWads2018} for references on the multivariate generalized Pareto distribution). The second building block is the extreme value copula (also called stable tail dependence function or STDF).\footnote{See e.g. \cite{Joe:1997}, \cite{Embrechts2000}, \cite{Beirlant:2004} and \cite{McNeilFreyEmbrechts05}.}

Broadly speaking, estimation of the STDF is divided in two approaches: parametric and semi-parametric. The former is based on parametric copula functions, the logistic and $t$ copulas are commonly used (see, for example, \cite{LoginSolnik01} for an application to extreme correlation of international equity markets, and \cite{CholletePenaLu11} for its use in investment diversification across major stock market indexes). The latter is based on higher order statistics (see \cite{Embrechts2000} for a theoretical treatment, and \cite{Straetmans04} for an application to asset market linkages in crisis periods).\footnote{\cite{LoginSolnik01} exploit, in the bivariate case, the explicit and simple relation between the tail dependence coefficient of the Gumbel copula and the linear correlation coefficient for extreme events, also known as exceedance correlation. In a similar vein, \cite{CizeauPottersBouchaud01} introduce the quantile correlation, i.e. the sample correlation between observations that are contained in a ball around a given joint quantile.} As pointed out in \cite{Straetmans08}, estimation of the STDF has the weakness that it presupposes tail dependence, besides that the parametric copula rests on parametric assumptions. An alternative, proposed by \cite{Ledford96}, consists of testing for tail dependence through the tail index of an auxiliary variable (the cross-sectional minimum of the random vector). \cite{Hartmann2005} uses it for studying the banking system, \cite{PoonRockingerTawn04} for estimating the tail dependence among risky asset returns, and \cite{Straetmans08} for studying US sectoral stock indexes around 9/11, respectively.
%The use of extreme value theory has, however, shortcomings. The main one is that the theory builds upon asymptotic results on the tails. Since in practice we estimate using a cut-off point of the tail, the asymptotic results are an approximation. Moreover, precise estimators require large sample sizes.

%\david{Tail dependence: This is too vague, it is not a measure but a statistical condition. The tail dependence coefficient (TDC) which is nothing else than an asymptotic conditional probability is only one of them. Tail dependence also implies that the unit contour lines representing the tail copula function are concave towards the origin. So, I would refer here to the tail dependence "coefficient" as a measure (but there are others). If it is nonzero there is tail dependence. Notice the tail beta is basically a special case of the TDC. The exact height of the TDC determines the STRENGTH of the tail dependence.}

%(also called extremal dependence structure and co-excedaance probability) steaming from extreme value theory (EVT henceforth) is the most used. The main building block is the assumption that tails asymptotically decay according to a power law that is governed by the tail index \david{Pareto-type tail declines are the main building block of univariate EVT, not multivariate EVT, I would say. It is true that the Ledford and Tawn approach also boils down to  mapping back joint probabilities into the univariate tail of some auxiliary variable Z whose tail index then reflects the degree of tail dependence (neta=1 or neta<1). But if you study extreme comovements with the stable tail dependence function (or "tail copula") no tail index is involved (cf. the framework to describe extremal comovements in my 2004 RESTAT). This is because neta=1 imposed in the latter framework. The estimator of the STDF in the 2004 RESTAT paper becomes degenerate under tail independence, that is why. De Vries (2005) in JBF ("the simple economics of bank fragility") offers an economic motivation for this tail dependence restriction.}.

%Broadly speaking, multivariate EVT is divided in two approaches: parametric and semi-parametric \david{the estimation approaches are falling into these two categories, not the statistical theory. Copulas can both be estimated using parametric techniques, i.e. imposing a logistic copula and applying ML lik in Ledford and Tawn) or with a semi-parametric estimator(see RESTAT 2004).}. The former is based on copula functions (see for instance \cite{McNeilFreyEmbrechts05} and \cite{HuaJoe11} for theoretical treatments, and \cite{CholletePenaLu11} for its use in investment diversification across major stock market indexes). The latter leaves unspecified the probability law at the extremes, which is generically explained by the so-called dependence function \david{the stable tail dependence function or tail copula approach means the same and as said, can be estimated by either imposing a parametric model or not.}. This function is, in general, unknown and depends on the tail index \david{This is not true (well, is is true in your tailcor framework but that is due to the fact you consider the universe of elliptical dfs). For example, the "dependence" parameter in the logistic model is NOT the tail index of the marginals which is normalized to 1 in the framework ("unit frechet"). The tail index only related to the tail dependence in specific circumstances, e.g. bivariate Pareto. }. To overcome this lack of knowledge, it is often assumed a logistic dependence function; see \cite{Ledford96}. Under this assumption, and in the bivariate case, \cite{LoginSolnik01} exploit the explicit and simple relation between the tail index \david{tail index: no, it is the logistic dependence parameter.}and the linear correlation coefficient for extreme events, also known as exceedance correlation.\footnote{In a similar vein, \cite{CizeauPottersBouchaud01} introduce the quantile correlation, i.e. the sample correlation between observations that are contained in a ball around a given joint quantile.} As pointed out in \cite{Straetmans08}, the dependence function \david{dependence function: stable tail dependence function" or "tail copula function"} has the weakness that it presupposes tail dependence, besides that the logistic assumption remains an approximation of the unknown dependence function. An alternative, proposed by \cite{Ledford96}, is based on the fact that the joint tail decay of a random vector is governed by the element of the vector that has the slowest tail decay. Hence estimating the tail decay of the cross-sectional minimum provides the coefficient of tail dependence. \cite{Straetmans08} denotes this method tail-$\beta$ \david{But you mix up here an estimation approach with the definition of the comovement indictor itself: the tail beta is a measure, not an estimation technique. There are at least 2 ways of estimating the tail beta using EVT estimation techniques: Either you could use the Ledford and Tawn approach indeed by not imposing tail dependence and estimating the tail index of the auxiliary variable Z (the tail dependence "parameter" neta). Alternatively, you can also use tail copula and thus impose tail dependence. Nonsurprisingly, you find that the latter tail betas exceed the former ones because of the tail dependence restriction.} and applies it to US sectoral stock indexes around 9/11. Similarly, \cite{PoonRockingerTawn04} explore the tail dependence structure among risky asset returns and present a framework for identifying joint tails using \cite{Ledford96}. The use of multivariate EVT has, however, shortcomings. The core of the theory builds upon asymptotic results on the tails. Since in practice we estimate using a cut-off point of the tail, the asymptotic results are an approximation. Moreover, the use of a power law hinders the analysis of tails that are equal or thinner than the Gaussian.
 
%Moreover in the context of extreme value theory, they are not able to disentangle between the linear and nonlinear correlations. This is however possible within copulas, but the analytical form heavily depends on the choice of the copula function. Moreover, in large dimensional problems only the Gaussian (which does not have tail dependence) and Student-$t$ copulas are realistic and feasible, while in vast dimensional problems only the Gaussian is feasible.

%\cite{LoginSolnik01} introduce the exceedance correlation, i.e. the sample correlation between observations that are jointly beyond a given threshold. In a similar vein, \cite{CizeauPottersBouchaud01} introduce the quantile correlation, i.e. the sample correlation between observations that are contained in a ball around a given joint quantile. These two measures are similar and, when applied to thresholds and quantiles that are far on the tails, the number of observations is limited, and large sample sizes are needed to obtain precise estimators.
%Moreover, these measures are not able to disentangle between the linear and nonlinear contributions.

While EVT-based literature is semi-parametric (in the sense that only the asymptotic tail is parametrized), another branch of the literature parametrises the whole distribution while assuming heavy tails -- see \cite{BLV} for a survey. The scale mixtures of multinormal distributions are particularly relevant since the elliptical and the normal mean-variance mixture distributions are used in this article. These distributions have the feature that the dependence between two random variables is given by the dispersion matrix and a single tail index (and the vector of skewness in the case of the normal mean-variance mixture). \cite{FW} proposes a new family of distributions, coined multiple scaled distributions, with the main feature that there are as many tail indexes as the dimension of the random vector. Another relevant fully parametric class of distributions are copulas, where the meta-elliptical copula of \cite{FangFangKotz2002} plays a dominant role. Beyond ellipticity, \cite{LeeLong} propose a multivariate conditional variance model that allows to model conditional correlation and dependence separately and simultaneously with nonelliptically distributed dependent errors.

\subsubsection*{This paper}

We introduce TailCoR, a measure for dependence that 
%can be implemented under mild assumptions. TailCoR
%does not depend on asymptotic (on the tail) assumptions. Moreover, it
can be computed under tails that are fatter, equal, or thinner than Gaussian. In a nutshell, TailCoR between two random variables is based on the projection of the two variables onto a line, and then a tail Inter Quantile Range is computed. 
%This lack of assumption of the thickness of the tails is particularly appealing as it allows relations on the tail that are explained by the linear correlation, as illustrated in the following simple example: two Gaussian random variables with linear correlation 0.99 are asymptotically (on the tail) independent but they are highly dependent for any finite tail probability level.
TailCoR has the following useful features: it is simple and no optimizations are needed, it performs well in small samples, and under ellipticity (i.e., the probability contours are ellipsoids) TailCoR disentangles easily between the above mentioned linear and nonlinear components.

%TailCoR is based on the following simple idea: if two random variables (properly standardized) are positively related (either linear and/or nonlinearly), most of the times the pairs of observations have the same sign, meaning that most of the dots (that represent the pairs) concentrate in the north-east and south-west quadrants of the scatter plot. Now, consider the 45-degree line that diagonally crosses these quadrants, and project all the dots on this line. Since the two random variables are positively related, the projected dots -- that are sitting on the 45-degree line -- are dispersed all over the line.\footnote{In the case of negative relation, the dots mostly concentrate in the north-west and south-east quadrants, and the projection is on the 135-degree line.} The degree of dispersion depends on the strength of the relation between the two random variables. If weak, the cloud of dots does not have a well defined direction and the projected dots are concentrated around the origin (recall that the variables are standardized); and hence the dispersion is small. By contrast, if the relation is strong, the cloud is stretched around the 45-degree line and the projected dots are very dispersed. Therefore the interquantile range of the projection is informative about the relation, either linear or nonlinear.


% the product of two components: one that only depends on the linear correlation coefficient and another that solely depends on the tail index. This is an appealing property of TailCoR that allows to disentangle the linear and nonlinear contributions. TailCoR has three further advantages: i) it is exact for any probability level as it is not based on tail asymptotic arguments, ii) it does not depend of any specific distributional assumption, iii) it is simple and no optimizations are needed. Moreover, the component that depends on the tail index may explain both heavy and thin tails (i.e. thinner than the Gaussian). Indeed, since the disentangling of TailCoR in the two contributions is under the elliptical family (but without imposing any specific distribution), the tails can be fatter, equal or thinner than those of the Gaussian distribution.

We also show an extension that differentiates between the downside and upside TailCoRs. It is often the case, like in risk management, that the interest lies in the tail of one region of the distribution, which leads to TailCoR when the probability contours are asymmetric.
%We show that TailCoR also disentangles easily between the linear and nonlinear correlations.
% (see e.g. \cite{MenciaSentana09} and \cite{Jondeau10}).

%In the second extension we show how to summarize the tail correlations of the random vector in a single number or, alternatively, the linear and nonlinear correlations into two numbers.

%It may be of interest to have a unique TailCoR for the entire random vector instead of pairwise measures.
%ii) Negative correlation: TailCoR as explained in the previous paragraph, is designed for positive relation as it projects the pairs of observations in the 45--degree line. A simple transformation makes it suitable for negative relation.
%iii) TailCoR under asymmetry. Though ellipticity is a very general and realistic assumption, in some cases observations show asymmetric probability contours. To cope with this possibility we explain how to disentangle TailCoR in the linear and nonlinear contributions under the normal mean-variance mixture distribution (see e.g. \cite{MenciaSentana09} and \cite{Jondeau10}). 
% show that this distribution generates asymmetric exceedance correlations.
%iv) Dynamic TailCoR: it is easy to extend the simplest estimator to the dynamic case.
%v) Multivariate TailCoR: the plain definition is for a pair of random variables but it can be extended to a random vector, yielding a matrix of TailCoRs.

The empirical illustration is on daily returns of 21 financial market indexes across the globe. Data runs from January 2000 to July 2020, and hence it incorporates the two crises mentioned at the beginning of the Introduction. For comparison purposes we compute the upper and lower exceedance correlations of \cite{LoginSolnik01}, and the parametric and non-parametric tail dependence coefficients (the former with a $t$ copula, and the latter as in \cite{Straetmans08}). Results show that TailCoR, exceedance correlations and tail dependence coefficients behave similarly.

%for the overall sample show that both the linear and nonlinear contributions matter.
%Moreover, TailCoR, exceedance correlation, and the tail dependence coefficient are highly related, which confirms that all the measures explain the same stylized fact.
To study the dynamic behaviour we use windows of 3 years. 
The estimated TailCoRs are in line with the financial and economic events that happened during the sample. TailCoR increases in crises periods, when global dependence increases, as it happened in 2007-2008 (and the aftermath) as well as recently because of COVID-19. 
%The gains of TailCoR in relatively small samples become apparent.
The evolution of the other metrics is heterogeneous. While the exceedance correlations could not be computed because of lack of extreme observations in the windows, the tail dependence coefficients move along with TailCoR though they show a greater deal of variability.
%This reflects the increasing concerns of tail events emerging from the Eurozone -- namely the fears of an exit of Greece from the euro, the political turmoil in Italy, and the financial bailout in Spain.
% -- that could trigger a domino effect all over the continent and the rest of the world.

%the euro area sovereign bond yields for the period 2002-2012. The Green Paper of the European \cite{Commission11} assesses the feasibility of common issuance of sovereign bonds (the Stability bonds) among the Member States of the euro area.\footnote{Other proposals, more elaborated, of pan--European bonds are the Blue bonds of \cite{Bruegel10}, the European safe bonds of \cite{ESB11}, the Safe bonds of the \cite{Safe11}, the synthetic Eurobonds of \cite{BeckUhligWagner11}, and the Eurobills of \cite{HellwigPhilippon11}.} Though the document does not set guidelines for the implementation, it mentions that the new bonds should be a pool. The most natural way of pooling is by means of a linear combination. If so, the correlations between them play an important role in order to determine the risks associated with the pooling. Over the years the linear contribution to TailCoR has decreased significantly since 2008. The average linear correlation coefficient before 2008 was close to 1 and at the end of the sample it was near 0.2. In other words, while before the crisis there was an almost perfect linear relation between the sovereign bond yields of the euro area, in 2009 it started to decreased, reaching in 2011 very low values, never seen before the creation of the common currency. This is in contrast with the non--linear contribution of TailCoR. It was very low from 2002 to 2007 but since them it has increased steadily, specially during the last two years. The backbone of this analysis is that the a common issuance of sovereign bonds by pooling sovereign bonds may have unexpected negative consequences for the peripheral and core countries, as they may not be necessarily less risky and more resilient to adverse shocks. A deeper analysis of the tail risks and tail correlations in the euro area sovereign bond yields can be found in \cite{Veredas12}.

The remaining sections are laid out as follows. Section 2 introduces the notation, assumptions, definition, and representations of TailCoR. It also shows a calibration exercise and the asymptotic properties of the estimators. Section 3 covers a brief Monte Carlo study. The extension to asymmetry is touched upon in Section 4.
%The implications for portfolio selection are described in Section 5, and 
The illustration to the market indexes is presented in Section 5. Section 6 concludes and proofs and lengthy tables are relegated to the appendixes.


==> RV_Methodology_JoE.tex <==
\section{TailCoR}

\subsection{Definition}

%\david{
%$Z=Y_j cos(g) + Y_k sin(g)$
%$Var(Z) = Var(Y_j)*(cos(g))^2 + Var(Y_j)*(sin(g))^2 + 2(cos(g)sin(g))Cov(Y_k,Y_j)$
%$Var(Z) = 1/k^2*(1+2(cos(g)*sin(g))\rho)$
%$IQR = s(alpha)*\sqrt{(1+2(cos(g)*sin(g))\rho)}$
%For g = pi*0.25 (45 degree line), 2(cos(g)*sin(g))=1. For g = pi*0.75 (135 degree line), 2(cos(g)*sin(g))=-1. For other values of g, |2(cos(g)*sin(g))|<1, and for g=pi*0.50, pi, pi*1.5, and pi=2, 2(cos(g)*sin(g))=0.
%In any case, the nonlinear correlation remains the same because under ellipticity the dependence on the tail is the same regardless of $\rho$.
%TO CHECK: if the estimator of s is the same regardless on the angle of the projection.} 

Let $\mathbf{X}_t$, $t=1,\ldots,T,$ be a random vector of size $N$ at time $t$ satisfying the following assumption
%\begin{itemize}
%\item[\bf G1] (a) $\mathbf{X}_1,\ldots,\mathbf{X}_T$ is a sequence of strongly stationarity random vectors. (b) $\mathbf{X}_t$ is $\phi$-mixing with $\phi(t)$ coefficients satisfying $\sum_{t-1}^{\infty} \phi(t)^{1/2}<\infty$.
%\end{itemize}

\begin{itemize}
\item[\bf G1] 
%\vspace{-0.2cm}
%\begin{itemize}
%\item[(a)]
(a) The random process $\left\{\mathbf{X}_t\right\}$ is a strongly stationary sequence of random vectors, (b) the unconditional distribution of $\mathbf{X}_t$ is unimodal, and (c)
%\item[(b)]
$\mathbf{X}_t$ is $S$-mixing.
%i.e. it satisfies the following two conditions: (i) for any $t $ and $m$, $P(|\mathbf{X}_t - \mathbf{X}_{tm}| \geq \gamma_m)\leq \delta_m$ for some numerical sequences $\gamma_m \rightarrow 0$, $\delta_m \rightarrow 0$, (ii) for any disjoint intervals $I_1,\ldots,I_r$ of integers and any positive integers $m_1,\ldots,m_r$, the vectors $\{\mathbf{X}_{tm_1},t\in I_1\},\ldots,\{\mathbf{X}_{tm_r},t\in I_r\}$ are independent provided the separation between $I_k$ and $I_l$ is greater than $m_k + m_l$.
%\end{itemize}
\end{itemize}

Assumption {\bf G1}(a) is standard in time series analysis and {\bf G1}(b) is due to \cite{Sherman55}. Both relate to the unconditional distribution of $\mathbf{X}_t$. Assumption {\bf G1}(c) relates to the conditional distribution and it specifies the time dependence of $\mathbf{X}_t$. The purpose of unimodality is twofold. First, it rules out distributions with several modes (but not asymmetry). Second, we consider the Gaussian and uncorrelated (hence independent) process as the benchmark. Regarding  {\bf G1}(c), assuming a mixing condition instead of a particular type of dynamic model makes TailCoR applicable to a wide array of processes. The conditions for $S$-mixing, introduced by \cite{BerkesHormannSchauer09}, apply to a large number of processes often used in economics and finance, including GARCH models and its extensions, linear processes (like ARMA models), and stochastic volatility among others. 
%The notation {\bf G} stands for General, as opposed to {\bf E} and {\bf A} for ellipticity and asymmetry that are used below.

TailCoR is based on the following simple idea, shown in Figure \ref{fig:scatterplots}. If two random variables $X_j$ and $X_k$ (properly standardized) are positively related (either linear and/or nonlinearly), most of the times the pairs of observations (depicted with circles) have the same sign, in the sense that most of them concentrate in the north-east and south-west quadrants of the scatter plot. Now, consider the $\phi$-degree line that crosses these quadrants (we illustrate the figure with $\phi=\pi/4$ or the 45-degree line) and project all the pairs on this line, producing a new random variable $Z^{(j\,k)}$, depicted with squares.\footnote{Because of representation purposes we show the projection only for the observations that are far from the origin, but the reader should keep in mind that the projection is done for all the observations.} Since the two random variables are positively related, the squares -- that are sitting on the $\phi$-degree line -- are dispersed all over the line.\footnote{In the case of negative relation, the dots mostly concentrate in the north-west and south-east quadrants, and the projection is on the corresponding $\phi$-degree line, as explained in detail later.} The extend of the dispersion depends on the strength of the relation between $X_j$ and $X_k$. If weak, the cloud of dots is concentrated around the origin without a well defined direction
%{\color{red} here is an important point I disagree with. Namely, what if one variable takes values on [-10,10], the other, say, on [-1,1], but they are not strongly correlated? These points will be far stretched out, despite lack of correlation. So this saying, that no correlation implies concentration around the center, has to be changed. Also, in the example that I mention, the line would obviously not be the 45-degree line, but rather the 0 degree line.}
The dispersion of the squares is therefore small. By contrast, if the relation is strong, the cloud of dots is stretched around the $\phi$-degree line, and hence the squares are very dispersed. 
%Therefore the dispersion of the projection is informative about the relation, either linear or nonlinear.

%\begin{center}[FIGURE \ref{fig:scatterplots} ABOUT HERE]\end{center}

\begin{figure}[!ht]
  \caption{Diagrammatic representation of TailCoR}
  \begin{center}
%  \vspace{0.2cm}
%    \includegraphics[angle=0,width=.5\linewidth]{Diagram1}
    \subfloat[Linear relation]{\includegraphics[angle=0,width=.45\linewidth]{Diagram-1}}
    \hspace{0.6cm}
    \subfloat[nonlinear relation]{\includegraphics[angle=0,width=.45\linewidth]{Diagram0}} \\
    \subfloat[Linear and nonlinear relation]{\includegraphics[angle=0,width=.45\linewidth]{Diagram}} \\
%    \hspace{0.6cm}
%    \subfloat[nonlinearity in the tails]{\includegraphics[angle=0,width=.45\linewidth]{Diagram4}} \\
%\begin{tabular}{p{8cm}} 
\begin{tabular}{p{14.5cm}}
\scriptsize Scatter plots where  $X_j$ and $X_k$ are positively related (the pairs are depicted with circles). Projecting the observations onto the $\phi$-degree line produces the random variable $Z^{(j\,k)}$, depicted with squares. Because of representation purposes we show the projection only for the observations on the tails but the reader should keep in mind that the projection is done for all the observations. Panel (a) shows the case of linear relation only. Panel (b) displays the case of nonlinear relation only. Panel (c) shows the scenario of both linear and nonlinear relations.
%{\color{red} I don't like the fact that Panel (c) shows exactly the same diamonds as Panel (b). This precisely would lead to believe that only the nonlinear part matters. Btw, the IQR on Panels (b) and (c) is exactly the same, which underlines this fact. Is that on purpose? I think this is a point that confuses my understanding of TailCoR. I cannot see the linear part playing any role in Panel (c).}
\\ 
\end{tabular}
  \end{center}
  \label{fig:scatterplots}
\end{figure}


%Figure \ref{fig:scatterplots} displays three diagrammatic representations that put forward the intuition behind TailCoR. They show scatter plots, along with the 45-degree line, where two elements of the random vector, $X_j$ and $X_k$, are positively related (the pairs are depicted with circles). Projecting the observations onto the 45-degree line produces a new random variable $Z^{(j\,k)}$, depicted with squares. Because of representation purposes we show the projection only for the observations far from the origin, but the reader should keep in mind that the projection is done for all the observations.

TailCoR is equal -- up to a normalization -- to the difference between the upper and lower tail quantiles of $Z^{(j\,k)}$. This {\it tail interquantile range} can be large because of two reasons. First, if $X_j$ and $X_k$ are highly linearly correlated (panel (a) of Figure \ref{fig:scatterplots}). Second, if the  correlation between $X_j$ and $X_k$ only happens on the tails, while the observations around the origin form a cloud with undefined direction (panel b). These two situations are not mutually exclusive and both may happen, which is actually the most likely case in practice (panel c). Either way, TailCoR is large, in a sense to be precisely defined below. But first we put this intuition at work.

%\footnote{Similar construction has been used by \cite{DominicyOgataVeredas12} for estimating the dispersion matrix of an elliptical distribution.}
%Moderate departures from linearity can also be handled by TailCoR, as shown in the bottom right scatter plot in which the relation between $X_j$ and $X_k$ appears to be U-shaped. The case where $X_j$ and $X_k$ are negatively related is treated in the next Section.

%\begin{figure}[!ht]
%  \caption{Diagrammatic representation of TailCoR}
%  \begin{center}
%%  \vspace{0.2cm}
%%    \includegraphics[angle=0,width=.5\linewidth]{Diagram1}
%    \subfloat[Linear correlation]{\includegraphics[angle=0,width=.45\linewidth]{Diagram-1}}
%    \hspace{0.6cm}
%    \subfloat[nonlinear correlation]{\includegraphics[angle=0,width=.45\linewidth]{Diagram0}} \\
%    \subfloat[Linear and nonlinear correlation]{\includegraphics[angle=0,width=.45\linewidth]{Diagram1}} \\
%%    \hspace{0.6cm}
%%    \subfloat[nonlinearity in the tails]{\includegraphics[angle=0,width=.45\linewidth]{Diagram4}} \\
%%\begin{tabular}{p{8cm}} 
%\begin{tabular}{p{14.5cm}}
%\scriptsize Scatter plots, along with the 45-degree line, where  $X_j$ and $X_k$ are positively related (the pairs are depicted with circles). Projecting the observations onto the 45-degree line produces the random variable $Z^{(j\,k)}$, depicted with squares. Because of representation purposes we show the projection only for the observations on the tails but the reader should keep in mind that the projection is done for all the observations Top left plot shows the case of only linear correlation. Top right plot displays the case of only nonlinear correlation. Bottom left shows the scenario of both linear and nonlinear correlation. Bottom right plot displays a situation where the relation on the tails is nonlinear. \\ 
%\end{tabular}
%  \end{center}
%  \label{fig:scatterplots}
%\end{figure}

Let $X_{j\,t}$ be the $j$th element of the random vector $\mathbf{X}_t$. Denote by $\mbox{Q}^{\tau}_j$ its $\tau$th quantile for $0<\tau<1$, and let $\mbox{IQR}^{\tau}_{j}=\mbox{Q}^{\tau}_j-\mbox{Q}^{1-\tau}_j$ be the $\tau$th interquantile range. A typical value of $\tau$ is 0.75. Let $Y_{j\,t}$ be the standardized version of $X_{j\,t}$:
\begin{equation}\label{eq:standard}
Y_{j\,t} = \frac{X_{j\,t} - \mbox{Q}^{0.50}_j}{\mbox{IQR}^{\tau}_{j}}.
\end{equation}
Likewise for $Y_{k\,t}$. In our context of potential heavy tails, the median and the interquantile range are used for the standardization. The mean of $Y_{j\,t}$ is not necessarily zero and its variance is not one, if they exist. This is not an issue since the aim of \eqref{eq:standard} is to have the pair $(Y_{j\,t},Y_{k\,t})$ centered around the same number and with the same scale. As \eqref{eq:standard} is based on marginal quantiles, we need the following technical assumption
\begin{itemize}
\item[\bf G2]  The random variable $X_{j\,t}$ has $F(x_{j})$ as cumulative distribution function  with density $f(x_{j})$ that is continuous and non-zero in a neighbourhood of $\mbox{Q}^{\tau}_j$ for $\tau \in [0,1]$. Likewise for $X_{k\,t}$.
%(a) For  $0<\tau<1$, the cumulative distribution function of $X_{j\,t}$ at point $x_{j\,t}$, denoted by $F(x_{j\,t})$, is continuous in some neighborhood of $\mbox{Q}^{\tau}_j$. (b) The probability density function at $x_{j\,t}$, denoted by $f(x_{j\,t})$, is such that $0<f(\mbox{Q}^{\tau}_j)<\infty$. Likewise for $X_{k\,t}$.
%\item[\bf G2] (a) For  $0<\tau<1$, the cumulative distribution function of $X_{j\,t}$ at point $x_{j\,t}$, denoted by $F(x_{j\,t})$, is continuous in some neighborhood of $\mbox{Q}^{\tau}_j$. (b) The probability density function at $x_{j\,t}$, denoted by $f(x_{j\,t})$, is such that $0<f(\mbox{Q}^{\tau}_j)<\infty$. Likewise for $X_{k\,t}$.
\end{itemize}

%Admittedly, TailCoR is best suited for situations when the tails of the marginal distributions are the same. Otherwise, TailCoR may increase when a marginal tail increases but the dependence between $X_{j\,t}$ and $X_{k\,t}$ does not change. In these cases, the effect of the marginal tails can be removed under 

Alternatively to \eqref{eq:standard}, $X_{j\,t}$ and $X_{k\,t}$ could be standardized with the marginal cumulative distribution functions, i.e. $Y_{j\,t}$ and $Y_{k\,t}$ would be the probability integral transforms that are distributed uniformly on $(0,1)$.
%(or a further transformation makes $Y_{j\,t}$ and $Y_{k\,t}$ unit Pareto).
This is advantageous if there are marginal dependencies beyond the location and the scale (like in the tails), or if we extend our method to copulas (as explained in the conclusions).
%Otherwise, as it is in the case of ellipticity discussed below, the standardisation \eqref{eq:standard} is enough.

By standard trigonometric arguments, the projection of $(Y_{j\,t},Y_{k\,t})$ on the $\phi$-degree line is
\begin{equation}\label{eq:proj}
%Z^{(j\,k)}_{t} = \frac{1}{\sqrt{2}}(Y_{j\,t} + Y_{k\,t}),
Z^{(j\,k)}_{t} = Y_{j\,t}\cos \phi + Y_{k\,t} \sin \phi,
\end{equation}
and the tail interquantile range of $Z^{(j\,k)}_{t}$ is
\begin{equation*}
\mbox{IQR}^{(j\,k)\,\xi}=\mbox{Q}^{(j\,k)\,\xi} - \mbox{Q}^{(j\,k)\,1-\xi},
\end{equation*}
where $\mbox{Q}^{(j\,k)\,\xi}$ is the $\xi$th quantile of $Z^{(j\,k)}_{t}$ and $\xi$ is typically beyond $0.90$.
%{\color{red} What is the reason for $\xi$ to be larger than $\tau$? We should explain it. To me it is not obvious}
The larger $\xi$ is, the further we explore the tails. We define TailCoR as follows.
\begin{description}
\item[{\bf Definition 1}] Under {\bf G1} -- {\bf G2}, TailCoR between $X_{j\,t}$ and $X_{k\,t}$ is
\begin{equation} \label{eq:definition}
%\mbox{TailCoR}^{(j\,k)\,\xi}  := S(\phi) s_g(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi},
\mbox{TailCoR}^{(j\,k)\,\xi}  := s_0(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi},
\end{equation}
%where $S(\phi)=1$ if $\phi \in [0,\pi/2)$ and $S(\phi)=-1$ if $\phi \in [\pi/2,\pi)$,
where $s_0(\xi,\tau)$ is a normalization such that under independence $\mbox{TailCoR}^{(j\,k)\,\xi}=1$, the reference value.
\end{description}

%\david{change the text of the normalization, which only applies to the elliptical case. Make general here and use the gaussian text for the elliptical case}

%First, $s_0(\xi,\tau)$ is the inverse of $\mbox{IQR}^{(j\,k)\,\xi}$ under independence. To compute it we either need a distributional assumption (as we do when assuming ellipticity) or Since this is a probability concept, some distributional assumption is needed. As explained later in detail, in the case of ellipticity, independence translates into Gaussianity and linear uncorrrelation. Once the Gaussianity and linear uncorrelation (and hence independence). Table \ref{tab:sg} in Appendix T shows values of $s_g(\xi,\tau)$ for a grid of reasonable values for $\tau$ and $\xi$. Alternatively, it can be computed as $s_g(\xi,\tau)=\frac{\Phi(\tau)^{-1}}{\Phi(\xi)^{-1}}$ where $\Phi(\cdot)$ is the cumulative distribution function of a standardized Gaussian distribution. 


%\david{the value of the normalization is computed for the case of elliptiticy (projection on the 45 or 135 degree lines? CHECK. If so, change the text}

%Interpolation can be used for values of $\xi$ and $\tau$ that are not in the table or, alternatively, a simple function can be programmed to compute exactly $s_g(\xi,\tau)$ for any value of $\tau$ and $\xi$. The steps for programming it are also given in Appendix T. %Second, $\mbox{TailCoR}^{(j\,k)\,\xi}$ does not depend explicitly on $\tau$, as it is chosen a priori for the standardization.
%Second, for the time being we deal with the bivariate definition, i.e. for the pair $(j\,k)$. The multivariate definition is treated below.

Four remarks are in order. First, the meaning of correlation in TailCoR is not the traditional one, as TailCoR is not bounded between -1 and 1, nor centered at zero. In the next sub-section, we deal with this issue in two ways. We first examine the bounds more in detail, and then we propose an alternative representation of TailCoR that is bounded between -1 and 1, and equals 0 under independence. 

Second, $ s_0(\xi,\tau)$ equals the inverse of the $\mbox{IQR}^{(j\,k)\,\xi}$ under independence. Also in the next sub-section, we show that in the case of ellipticity, the $\mbox{IQR}^{(j\,k)\,\xi}$ can be computed from a standard Gaussian distribution.

Third, TailCoR is not an asymptotic (in the tail) dependence measure. Instead, the dependence between $X_{j\,t}$ and $X_{k\,t}$ can be computed precisely for any $\xi$, and, since TailCoR does not rely on assumptions of the asymptotic behavior of the tail, it can be used for distributions with tails that are Pareto, exponential, or even with finite end points.

%The Gaussian distribution is a case in point. Suppose that the linear correlation between $X_{j\,t}$ and $X_{k\,t}$ is 0.99. While standard multivariate extreme value methods would conclude that $X_{j\,t}$ and $X_{k\,t}$ are asymptotically (in the tail) independent, TailCoR concludes that they are dependent for all $\xi <1$. Of course the Guassian 

%Extreme Value Theory \cite{PoonRockingerTawn04}

%Fourth, $\mbox{TailCoR}^{(j\,k)\,\xi}$ is also valid even for skewed and heavy tailed processes, for which the first and second moment may do not exist, provided that the random process is $S$-mixing and strongly stationary process.
Last, the angle $\phi$ has to be chosen. An optimality criterion would be to choose the angle between $0$ and $\pi$ that maximizes the $\mbox{IQR}^{(j\,k)\,\xi}$. In practice this can be done with a grid search on $\phi$, computing the projection and the tail interquantile range for each angle of the grid. Since no optimizations are involved, this grid search is computationally inexpensive. 


%as it is done in the next sub-section.
%Last, though the standardization puts the two random variables in the same scale, and hence aligned with the 45-degree line, the projection into another $\gamma$-degree line is $Z^{(j\,k)}_{t} = Y_{j\,t}\cos \gamma + Y_{k\,t}\sin \gamma$.


\subsection{Disentangling the linear and nonlinear components}

\subsubsection*{Ellipticity and assumptions}

Though definition (\ref{eq:definition}) is simple and intuitive, it does not allow to understand how much of TailCoR is due to the linear and nonlinear dependencies. This is possible however if we assume ellipticity.
\begin{itemize}
\item[\bf E1] The unconditional distribution of $\mathbf{X}_t$ belongs to the elliptical family, given by the stochastic representation $\mathbf{X}_t =_d \bm{\mu} + \mathcal{R}_{\alpha\,t}\bm{\Lambda}\mathbf{U}_t$.
\end{itemize}
%The notation {\bf E} stands for Elliptical.
The $N \times 1$ random vector $\mathbf{U}_t$ under {\bf E1} is uniformly distributed on the unit sphere. The scaling matrix $\bm{\Lambda}$ produces the ellipticity and is such that $\bm{\Sigma}=\bm{\Lambda} \bm{\Lambda}^{\prime }$, a positive definite symmetric dispersion matrix -- often called the shape matrix with generic $(j\,k)$ element $\sigma_{X_j\,X_k}$, and for convenience we denote the $(j\,j)$ diagonal element by $\sigma_{X_j}^2$. The non-negative and continuous random variable $\mathcal{R}_{\alpha\,t}$ generates the tail thickness through a so-called radial density depending on the shape parameter $\alpha$, and is stochastically independent of $\mathbf{U}_t$. From now on, we will denote $\alpha$ as the tail index, in the sense that this parameter explains the decay of the tails (the smaller $\alpha$ the thicker the tails), but not necessarily according to a power law.\footnote{The random variable $\mathcal{R}_{\alpha\,t}$ may not only depend on the tail index but on a vector of shape parameters. We do not consider the latter since most of the elliptical distributions used in practice only depend on $\alpha$ (see examples after assumption {\bf E2}). The extension is however straightforward.} The vector $\bm{\mu}$ re-allocates the center of the distribution. Let $\bm{\theta}=(\bm \mu, \bm \Sigma, \alpha) \in \bm\Theta$ denote the vector of unknown parameters satisfying the following standard assumption.
\begin{itemize}
\item[\bf E2] (a) The parameter space $\bm{\Theta}$ is a non-empty and compact set on $\mathbb{R}^{N+\frac{N(N+1)}{2}+1}$. (b) The true parameter value $\bm{\theta}_0$ belongs to the interior of $\bm{\Theta}$.
\end{itemize}

Note that assumption {\bf E1} implies that the unconditional distribution of $\mathbf{X}_t$ belongs to the elliptical family, but no specific distributional assumption is made. The elliptical family nests, among others, the Gaussian, Student-$t$, elliptical stable (ES henceforth), Cauchy, Laplace, power exponential, and Kotz probability laws.\footnote{See \cite{Hashorva08} and \cite{Hashorva10} for tail theory within the elliptical family.} For a given vector of locations and a dispersion matrix, the difference between two elliptical distributions is the random quantity $\mathcal{R}_{\alpha\,t}$ with tail index $\alpha$, which plays a central role here. Another feature of the elliptical family is its closeness under location and scale shifts, which implies that $Z_t^{(j\,k)}$ is elliptical with the same tail index $\alpha$.

We further need the existence of the mean and the variance-covariance matrix:
\begin{itemize}
\item[\bf E3] The unconditional moments up to order 2 are finite, i.e. $E(\mathbf{X}_t^p) < \infty, \mbox{ for } p \leq 2$.
\end{itemize}
%This assumption implies that the mean, the variance-covariance matrix, and the correlation matrix are $E(\mathbf{X}_t) = \bm{\mu}$,
%$Cov(\mathbf{X}_t) = E(\mathcal{R}_{\alpha})\bm{\Sigma}$, and 
%$Corr(\mathbf{X}_t) = diag(\bm{\Sigma})^{-1/2}\bm{\Sigma}diag(\bm{\Sigma})^{-1/2}$.
%Note that the correlation matrix, with $(j\,k)$ element $\rho_{j\,k}$, does not depend on the tail index.

%This is very general and covers many cases encountered in practical work.
%It does not cover however the cases like the bottom right scatter plot of Figure \ref{fig:scatterplots} as the probability contours are not elliptical.

%This assumption may be relaxed, as explained in the estimation section
Next, we substitute assumptions {\bf G1} and {\bf G2} for

\begin{itemize}
\item[\bf E4] (a) The random process $\left\{\mathbf{X}_t\right\}$ is a weakly stationary sequence of random vectors, and (b) $\mathbf{X}_t$ is $S$-mixing.
%, i.e. it satisfies the following two conditions: (i) for any $t $ and $m$, $P(|\mathbf{X}_t - \mathbf{X}_{tm}| \geq \gamma_m)\leq \delta_m$ for some numerical sequences $\gamma_m \rightarrow 0$, $\delta_m \rightarrow 0$, (ii) for any disjoint intervals $I_1,\ldots,I_r$ of integers and any positive integers $m_1,\ldots,m_r$, the vectors $\{\mathbf{X}_{tm_1},t\in I_1\},\ldots,\{\mathbf{X}_{tm_r},t\in I_r\}$ are independent provided the separation between $I_k$ and $I_l$ is greater than $m_k + m_l$.
\item [\bf E5] The random variable $\mathcal{R}_{\alpha\,t}$ has $P(r)$ as  cumulative distribution function   with density $p(r)$ that is  continuous and non-zero in a neighbourhood of $\mbox{Q}^{\tau}_j$ for $\tau \in [0,1]$.
\end{itemize}

%Assumption {\bf E5} replaces {\bf G2} since it ensures that the marginal distributions of the elements of $\mathbf{X}_t$ fulfill the conditions in {\bf G2}.

\subsubsection*{The optimal projection}

Ellipticity allows to compute the optimal angle $\phi$ without the grid search mentioned above. The interquantile range used in the standardization \eqref{eq:standard} can be written as $k(\tau,\alpha)\sigma_{X_j}$, where $k(\tau,\alpha)$ is a non-random positive constant. Likewise $\mbox{IQR}^{\tau}_{k}=k(\tau,\alpha)\sigma_{X_k}$.\footnote{\cite{McC1986} introduced this relation between the IQR and the scale parameter in the context of stable distributions.} Then, by {\bf E1} the bivariate random vector $Y^{j\,k}_t=(Y_{j\,t},Y_{k\,t})$ is elliptically distributed with a $2 \times 2$ shape matrix $k(\tau,\alpha)^{-2}\bm{\mbox{R}}$. The matrix $\bm{\mbox{R}}$ has diagonal elements $\rho_{11}=\rho_{22}=1$ and off diagonal element $\rho_{12}=\sigma_{X_j\,X_k}/\sigma_{X_j}\sigma_{X_k}$ (3.3.2 of \cite{McNeilFreyEmbrechts05}).

The probability contours of $Y^{j\,k}$ are therefore ellipsoids with axes that are in the direction of the eigenvectors of $k(\tau,\alpha)^2\bm{\mbox{R}}^{-1}$, and their lengths are proportional to the reciprocals of the square roots of the eigenvalues of $k(\tau,\alpha)^2\bm{\mbox{R}}^{-1}$. Since $\rho_{11}=\rho_{22}=1$, the first eigenvalue is $k(\tau,\alpha)^{-2}(1+\rho_{12})$ with associated eigenvector $(1/\sqrt{2},1/\sqrt{2})$, while the second eigenvalue is $k(\tau,\alpha)^{-2}(1-\rho_{12})$ with associated eigenvector $(1/\sqrt{2},-1/\sqrt{2})$.

If the relation between $X_{j\,t}$ and $X_{k\,t}$ is positive, then $\rho_{12}$ is positive and $k(\tau,\alpha)^{-2}(1+\rho_{12})$ is the largest eigenvalue. Hence the projection on the 45-degree line is optimal:
\begin{equation}\label{eq:proj}
Z^{(j\,k)}_{t} = \frac{1}{\sqrt{2}}(Y_{j\,t} + Y_{k\,t}).
\end{equation}
If $\rho_{12}$ is negative, then $k(\tau,\alpha)^{-2}(1-\rho_{12})$ is the largest eigenvalue and the projection in the 135-degree line is optimal:
\begin{equation}\label{eq:proj}
Z^{(j\,k)}_{t} = \frac{1}{\sqrt{2}}(Y_{j\,t} - Y_{k\,t}).
\end{equation}
Either way, $Z^{(j\,k)}_{t}$ is the first principal component of $Y^{j\,k}$. The choice between the 45- and the 135-degree lines depends on the sign of $\rho_{12}$. If wrongly chosen, conclusions may be misleading, as exemplified in Figure \ref{fig:negtailcor}.
%\subsection*{Negative correlation}
%$\mbox{TailCoR}^{(j\,k)\,\xi}$, as defined so far, is designed for positive relations as it projects the pairs of observations onto the 45-degree line.
Panel (a) shows the projection on the 45-degree line when the relation is negative. The projection $Z^{(j\,k)}$ is concentrated around the origin and $\mbox{TailCoR}^{(j\,k)\,\xi}$ can even be smaller than one, leading to the false conclusion that tails are thinner than Gaussian.
%{\color{red} where did we say that TailCoR <1 implies this? That is an important missing point! OK I see it comes later. We should indicate this here.}
Projecting on the 135-degree line, as shown in panel (b), captures correctly the negative relation between $X_{j\,t}$ and $X_{k\,t}$.

%\begin{center}[FIGURE \ref{fig:negtailcor} ABOUT HERE]\end{center}


\begin{figure}
  \caption{A diagrammatic representation of TailCoR for negative relation}\label{fig:negtailcor}
  \begin{center}
    \subfloat[Projection in the 45-degree line]{\includegraphics[angle=0,width=.45\linewidth]{Diagram2}}
    \hspace{0.6cm}
    \subfloat[Projection in the 135-degree line]{\includegraphics[angle=0,width=.45\linewidth]{Diagram3}} \\
\begin{tabular}{p{14.5cm}}
\scriptsize Scatter plots where $X_j$ and $X_k$ are negatively related and the projection is done with the wrong and right angles (panels (a) and (b) respectively).\\
% (the pairs are depicted with circles). Projecting the observations onto the 45- or 135-degree lines produces the random variable $Z^{(j\,k)}$, depicted with squares. \\ 
\end{tabular}
  \end{center}
\end{figure}

%In practice, we suggest the following simple algorithm for choosing between the 45- and the 135-degree lines, which is based on the fact that under independence the IQRs of both projections are the same. Let $Z^{(j\,k)}_{45\,t}$ and $Z^{(j\,k)}_{135\,t}$ be the corresponding projections. If $\mbox{IQR}^{(j\,k)\,\xi}_{45}>\mbox{IQR}^{(j\,k)\,\xi}_{135}$  then $Z^{(j\,k)}_{45\,t}$ is used, otherwise $Z^{(j\,k)}_{135\,t}$ is selected.

%A simple transformation makes $\mbox{TailCoR}^{(j\,k)\,\xi}$ suitable for negative relations. Instead of projecting onto the 45-degree line, we project onto the 135-degree line, as depicted in the right plot of Figure \ref{fig:negtailcor}. Following similar trigonometric arguments as before, the projection is now
%\begin{equation*}
%Z^{(j\,k)}_{t} = \frac{1}{\sqrt{2}}(Y_{j\,t} - Y_{k\,t}).
%\end{equation*}
%Under {\bf G1}-{\bf G2}, the definition remains, i.e. $\mbox{TailCoR}^{(j\,k)\,\xi} := s_g(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi}$. However, under {\bf E1}-{\bf E5}, the expression is slightly modified:
%\begin{equation*}
%\mbox{TailCoR}^{(j\,k)\,\xi} = s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt {1-\rho_{j\,k}}.
%\end{equation*}
%
%The proof of this result is not shown as it follows trivially from Theorem 1. The asymptotic distributions of Theorem 2 and the Corollary above are not modified.
%The projection onto the 45- or 135-degree line depends on the relation between the random variables. Let $Z^{(j\,k)}_{45\,t}$ and $Z^{(j\,k)}_{135\,t}$ be the corresponding projections. By noting that under independence the IQRs of both projections are the same, the following simple rule applies: if $\mbox{IQR}^{(j\,k)\,\xi}_{45}>\mbox{IQR}^{(j\,k)\,\xi}_{135}$  then $Z^{(j\,k)}_{45\,t}$ is used, otherwise $Z^{(j\,k)}_{135\,t}$ is selected.



%The following automatized algorithm for choosing the projection can be used. It is based on the fact that under independence the IQRs of both projections are the same:
 %Projecting onto the 45- or 135-degree line is a user choice. Visual inspection of the scatter plots for choosing the projection is only feasible when $\mathbf{X}_t$ is small dimensional. For vast dimensions we propose
%the following automatized method can be used for choosing the projection.
% for the pair $(j\,k)$, and let $\mbox{IQR}^{(j\,k)\,\xi}_{45}$
%and $\mbox{IQR}^{(j\,k)\,\xi}_{135}$ be the corresponding IQRs.
%If $\mbox{IQR}^{(j\,k)\,\xi}_{45}=\mbox{IQR}^{(j\,k)\,\xi}_{135}$ there is neither linear nor nonlinear correlation and $\mbox{TailCoR}^{(j\,k)\,\xi}$ computed in either way gives the same result.



\subsubsection*{TailCoR under ellipticity}

We are now ready to disentangle $\mbox{TailCoR}^{(j\,k)\,\xi}$ into the linear and nonlinear components.

\begin{description}
\item[{\bf Theorem 1}] Let $X_{j\,t}$ and $X_{k\,t}$ be two elements of the random vector $\mathbf{X}_t$ that fulfills assumptions {\bf E1} -- {\bf E5}. Let $\rho_{j\,k}$ be the linear correlation, and let $s(\xi,\tau,\alpha)$ be a continuous and monotonically decreasing function of $\alpha$. Then
\begin{equation*}
\mbox{TailCoR}^{(j\,k)\,\xi} = s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt{1+|\rho_{j\,k}|},
\end{equation*}
where $s_g(\xi,\tau)$ is a normalization such that under independence $\mbox{TailCoR}^{(j\,k)\,\xi}=1$, the reference value.

\end{description}

\begin{description}
\item[{\bf Proof}] See Appendix P.
\end{description}

The rightmost element, $\sqrt{1+|\rho_{j\,k}|}$, captures the linear dependency to $\mbox{TailCoR}^{(j\,k)\,\xi}$, while $s(\xi, \tau,\alpha)$ captures the nonlinear dependency as it depends on the tail index $\alpha$. We denote these dependencies as linear and nonlinear components.

The normalization has become now $s_g(\xi,\tau)$ where the subindex $g$ is for Gaussianity. Indeed, under ellipticity, independence translates into Gaussianity and linear uncorrelation and hence $s_g(\xi,\tau)=\frac{\Phi^{-1}(\tau)}{\Phi^{-1}(\xi)}$ where $\Phi(\cdot)$ is the cumulative distribution function of a standardized Gaussian distribution.\footnote{This can be shown using results of Theorem 1. Under Gaussianity and linear uncorrelation, $Z^{(j\,k)}_{t} \sim \frac{1}{2\Phi^{-1}(\tau)} N(0,1)$. Hence $\mbox{IQR}^{(j\,k)\,\xi}= \frac{\Phi^{-1}(\xi)}{\Phi^{-1}(\tau)}$. Since $s_g(\xi,\tau)\mbox{IQR}^{(j\,k)\,\xi}=1$, then $s_g(\xi,\tau)=\frac{\Phi^{-1}(\tau)}{\Phi^{-1}(\xi)}$.} Table \ref{tab:sg} in Appendix T shows values of $s_g(\xi,\tau)$ for a grid of reasonable values for $\tau$ and $\xi$.
%{\color{red} this is also not obvious to me. Where does this come from?}  

\begin{figure}
  \begin{center}  \caption{Sensitivity of $s_g(\xi,\tau)s(\xi,\tau,\alpha)$ to $\alpha$ and $\rho$}\label{fig:nonlinear}
  \vspace{0.5cm}
\subfloat[Sensitivity to $\alpha$]{\includegraphics[angle=0,width=0.43\linewidth]{S_student_changealpha}}
%\subfloat[Sensitivity to $\alpha$ - ES]{\includegraphics[angle=0,width=0.4\linewidth]{S_ES_changealpha}} \\
\subfloat[Sensitivity to $\rho$]{\includegraphics[angle=0,width=0.42\linewidth]{F_changerho}}\\
\begin{tabular}{p{12.5cm}}
\scriptsize Panel (a) shows the sensitivity of the nonlinear component to $\alpha$. The tail index varies from 2.5 to 30. Panel (b) shows the sensitivity to $\rho$ (for $\alpha=2.5$). Both plots are for $\tau=0.75$ and $\xi=0.95$.\\ 
\end{tabular}
  \end{center}
\end{figure}

Panel (a) of Figure \ref{fig:nonlinear} displays $s_g(\xi, \tau)s(\xi, \tau,\alpha)$ as a function of $\alpha$ and assuming a Student-$t$ distribution (and for $\xi=0.95$ and $\tau=0.75$). The tail index varies from 2.5 to 30. The nonlinear component decreases as $\alpha$ increases, and $s_g(\xi, \tau)s(\xi, \tau,\alpha)$ approaches  1 as $\alpha$ goes to $30$, or when the distribution is indistinguishable from the Gaussian. 
%The table in Appendix T shows that $s_g(0.95,0.75)=0.41$, the inverse of 2.43, and hence $s_g(\xi, \tau)s(\xi, \tau,\alpha) \approx 1$ for $\alpha$ beyond $30$.
%Similar reading applies for the right plot, with a tail index that varies between 1.2 and 2. The decrease is more slow than for the Student-$t$ as tails remain significantly thicker than the Gaussian even for $\alpha$ in the vicinity of 2. 
Panel (b) shows the sensitivity of $s_g(\xi, \tau)s(\xi, \tau,\alpha)$ to $\rho$ (with $\alpha=2.5$).
%under the Gaussian (solid line) and Student-$t$ (dashed line) distributions.
The nonlinear component is not affected by $\rho$, which confirms that $\sqrt{1+|\rho_{j\,k}|}$ and $s(\xi, \tau,\alpha)$ capture different aspects of $\mbox{TailCoR}^{(j\,k)\,\xi}$.

%\begin{center}[FIGURE \ref{fig:nonlinear} ABOUT HERE]\end{center}

%\begin{figure}[!h]
%  \begin{center}  \caption{Sensitivity of $s(\xi,\tau,\alpha)$ to $\alpha$ and $\rho$}\label{fig:nonlinear}
%  \vspace{0.5cm}
%\subfloat[Sensitivity to $\alpha$ -- Student-$t$]{\includegraphics[angle=0,width=0.4\linewidth]{S_student_changealpha}}
%\subfloat[Sensitivity to $\alpha$ -- ES]{\includegraphics[angle=0,width=0.4\linewidth]{S_ES_changealpha}} \\
%\subfloat[Sensitivity to $\rho$]{\includegraphics[angle=0,width=0.4\linewidth]{F_changerho}}\\
%\begin{tabular}{p{12.5cm}}
%\scriptsize The top plots show the sensitivity of the nonlinear correlation to $\alpha$ for the Student-$t$ (left) and ES (right) distributions. For the Student-$t$ the tail index varies from 2.5 to 30 while for the ES it varies from 0 to 2. The bottom plot shows the sensitivity to $\rho$ (which takes the full range $[-1,1]$) for the Gaussian (solid line) and the Student-$t$ (dashed line) distributions. All the plots are for $\tau=0.75$ and $\xi=0.95$.\\ 
%\end{tabular}
%  \end{center}
%\end{figure}

$\mbox{TailCoR}^{(j\,k)\,\xi}$ has numerous properties.
%First, it is location-scale invariant, i.e. $\mbox{TailCoR}^{(j\,k)\,\xi}$ between $X_{j\,t}$ and $X_{k\,t}$ is the same as between $a + bX_{j\,t}$ and $c+dX_{k\,t}$, for $a,b,c$, and $d$ real numbers.
First, it captures nonlinear dependencies if tails deviate from Gaussianity,
%I.e. if tails are fatter, equal or thinner than those of the Gaussian distribution,
i.e. $s(\xi,\tau,\alpha)s_g(\xi,\tau)$ can be greater, equal, or smaller than 1 (corresponding to tails fatter, equal or thinner than the Gaussian distribution). 
%is larger than one as $s_g(\xi,\tau)s(\xi,\tau,\alpha)>1$,\footnote{This is akin to the coefficients of tail dependence steaming from copula theory. For instance, for the bivariate case, the coefficient of tail dependence of a Student-$t$ copula is $2 t_{\alpha+1}\left(-\sqrt{\frac{(\alpha+1)(1-\rho)}{1+\rho}}\right)$, where $t_{\alpha+1}(\cdot)$ is a standardized Student-$t$ cumulative distribution function with tail index $\alpha+1$. Even if $\rho=0$ the tail dependence is positive.} and iii) $\mbox{TailCoR}^{(j\,j)\,\xi}=s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt{2}$.
%, and iii) $\mbox{TailCoR}^{(j\,j)\,\xi}$, i.e.  between $X_j$ and itself, is $\sqrt{2}$. If, by contrast, $\mathbf{X}_t$ is heavy tailed, i) $s(\xi,\tau,\alpha)$ captures the nonlinear correlation: the heavier tailed $\mathbf{X}_t$ is, the higher is $s(\xi,\tau,\alpha)$ and so does $\mbox{TailCoR}^{(i\,j)\,\xi}$,
%This term is estimated rather than tabulated, as explained below.
Second, even if $X_j$ and $X_k$ are linearly uncorrelated, $\mbox{TailCoR}^{(j\,k)\,\xi}$ is different from 1 if $X_j$ and $X_k$ are non-Gaussian. This is akin to the coefficient of tail dependence stemming from copula theory.\footnote{For instance, the tail dependence coefficient of a bivariate Student-$t$ copula is $2 t_{\alpha+1}\left(-\sqrt{\frac{(\alpha+1)(1-\rho)}{1+\rho}}\right)$, where $t_{\alpha+1}(\cdot)$ is a standardized Student-$t$ cumulative distribution function with tail index $\alpha+1$. Even if $\rho=0$ tail dependence is positive (unless $\alpha \rightarrow \infty$).} Third, if 
%As for the remaining properties, for the ease of exposition we consider two cases: either $\mathbf{X}_t$ is thin tailed (i.e. Gaussian) or heavy tailed. If
$\mathbf{X}_t$ is Gaussian, $s(\xi,\tau,\alpha)s_g(\xi,\tau)=1$ and $\mbox{TailCoR}^{(j\,k)\,\xi} = \sqrt{1+|\rho_{j\,k}|}$, \mbox{i.e.} the only source of dependence is linear.
%{\color{red} I know this was already said, but how can we actually see this? I mean, yes, we did it via Figure 3, but I would like to see some theoretical argument here. Probably obvious and I miss it}

This last property shows that under Gaussianity the upper bound is $\sqrt{2}$. Otherwise, the upper bound depends on $\alpha$ and $\xi$.
%In other words, on the value of the nonlinear correlation.
Figure \ref{fig:nonlinear2} displays similar curves to those in panel (a) of Figure \ref{fig:nonlinear} for values of $\xi$ typically used in practice: 0.90 (solid line), 0.95 (thick dashes), 0.975 (thin dashes), and 0.99 (thick and thin dashes). The further we explore the tails, the larger is $s_g(\xi, \tau)s(\xi, \tau,\alpha)$, and so is TailCoR. The range of values is $1-1.5$ (except if $\xi$ is close to 1 and tails are very heavy), which in turn translates into a range of values of TailCoR between 1 and 2.12 (e.g., if $\rho=1$, TailCoR equals $\sqrt{2}\times 1.5=2.12$).
%(the latter is for $\rho=1$ and $s_g(\xi, \tau)s(\xi, \tau,\alpha)$=1.3).

\begin{figure}
  \begin{center}\caption{Sensitivity of $s_g(\xi,\tau)s(\xi,\tau,\alpha)$ to $\alpha$ and $\xi$}\label{fig:nonlinear2}
\includegraphics[angle=0,width=0.6\linewidth]{S_student_changealphaxi}
\begin{tabular}{p{9cm}} 
\scriptsize Sensitivity of the nonlinear correlation to $\alpha$ for the Student-$t$ distribution. The tail index varies from 2.5 to 30. Each line is for a value of $\xi$: 0.90 (solid line), 0.95 (thick dashes), 0.975 (thin dashes) and 0.99 (thick and thin dashes).\\ 
\end{tabular}
  \end{center}
\end{figure}

We close this section with the issue that TailCoR is not a correlation in the traditional sense, as it is not centered at zero nor bounded above. A simple transformation consisting on subtracting 1, scaling by the value of TailCoR under perfect correlation, and multiplying by the sign of the correlation, leads to the following alternative expression
%\begin{eqnarray}\label{eq:alternative}
%\mbox{TailCoR}^{(j\,k)\,\xi}_{alt} &=& \mbox{sign}(\rho_{j\,k})\tanh(\mbox{TailCoR}^{(j\,k)\,\xi}-1) \quad \mbox{for $s_g(\xi,\tau)s(\xi,\tau,\alpha) \geq 1$}\\
%						 &=& (1-\mbox{sign}(\rho_{j\,k}))\tanh(\mbox{TailCoR}^{(j\,k)\,\xi}-1) \quad \mbox{for $s_g(\xi,\tau)s(\xi,\tau,\alpha) < 1$} \nonumber
%\end{eqnarray}
%where $\tanh$ is the hyperbolic tangent function, and $\mbox{sign}(\rho_{j\,k})=1$ if $\rho_{j\,k} \geq 1$ or 0 otherwise.
\begin{equation}\label{eq:alternative}
\mbox{TailCoR}^{(j\,k)\,\xi}_{alt} = \mbox{sign}(\rho_{j\,k})\frac{\mbox{TailCoR}^{(j\,k)\,\xi} - 1}{s_g(\xi, \tau)s(\xi, \tau,\alpha)\sqrt{2} - 1},
\end{equation}
which is bounded above and below by 1 and -1 and centered around 0, provided that TailCoR is larger than one. TailCoR smaller than one is pathological, as it occurs when tails are extremely light or when tails are light and the linear correlation is very low.

The only cases when $\mbox{TailCoR}^{(j\,k)\,\xi}_{alt}$ can be used even if TailCoR is smaller than one is when $X_{j\,t}$ and $X_{k\,t}$ are perfectly correlated. Then, $|\rho_{j\,k}|=1$ and \eqref{eq:alternative} equals 1 if $\rho_{j\,k}=1$, and -1 if $\rho_{j\,k}=-1$ regardless of the value of TailCoR.

If $\rho_{j\,k}=0$, \eqref{eq:alternative} becomes (assuming $\mbox{sign}(\rho_{j\,k})=1$ for $\rho_{j\,k}=0$)
\begin{equation*}
\mbox{TailCoR}^{(j\,k)\,\xi}_{alt} = \frac{s_g(\xi,\tau)s(\xi,\tau,\alpha) - 1}{s_g(\xi, \tau)s(\xi, \tau,\alpha)\sqrt{2} - 1},
\end{equation*}
which is zero only under Gaussianity; otherwise it is between -1 and 1.
%{\color{red} I do not see this. OK, if $s_g*s$ is larger than 1, then we have a bound of 1. Fine. But what if $s_g*s=0.1$? Then we get -0.9/(-0.86)>1}

\begin{figure}
  \begin{center}\caption{Alternative TailCoR}\label{fig:altTailCoR}
\includegraphics[angle=0,width=0.8\linewidth]{AlternativeTailCoR_eq}
\begin{tabular}{p{9cm}} 
\scriptsize Sensitivity of $\mbox{TailCoR}^{(j\,k)\,\xi}_{alt}$ (vertical axis) to values of $s_g(\xi,\tau)s(\xi,\tau,\alpha)$ (horizontal axis) and $\rho_{j\,k}$ (different lines)\\ 
\end{tabular}
  \end{center}
\end{figure}

Figure \ref{fig:altTailCoR} shows the value of $\mbox{TailCoR}^{(j\,k)\,\xi}_{alt}$ for different choices of $s_g(\xi,\tau)s(\xi,\tau,\alpha)$ and $\rho_{j\,k}$. The nonlinear component is in the horizontal axis and the nine lines represent values of $\rho_{j\,k}$: $\{1, 0.9, 0.5, 0.1, 0, -0.1, -0.5, -0.9, -1\}$. The horizontal solid lines at 1 and -1 are for $\rho_{j\,k}$ equal to 1 and -1 respectively, confirming what was mentioned above. As $\rho_{j\,k}$ gets closer to zero, the alternative TailCoR decreases, reaching zero when $s_g(\xi,\tau)s(\xi,\tau,\alpha)=1$ and $\rho_{j\,k}=0$ as represented by the grey dot. Note that, as explained earlier, $\mbox{TailCoR}^{(j\,k)\,\xi}_{alt}$ is not available for very light tails (e.g., $s_g(\xi,\tau)s(\xi,\tau,\alpha) \leq 0.5$ in the figure) or a combination of light tails and low correlation (e.g., $s_g(\xi,\tau)s(\xi,\tau,\alpha) = 0.9$ and $\rho_{j\,k}=0.1$ in the figure).


%If $|\rho_{j\,k}|<1$, 
%Under Gaussianity \eqref{eq:alternative} simplifies to
%\begin{equation}
%\mbox{TailCoR}^{(j\,k)\,\xi}_a = \mbox{sign}(\rho_{j\,k})\frac{\sqrt{1+|\rho_{j\,k}|} - 1}{\sqrt{2} - 1},
%\end{equation}
%which takes values -1, 0 and 1 if $\rho_{j\,k}$ equals -1, 0 and 1 respectively. 


%ii) the most appealing property is that, even if $X_j$ and $X_k$ are linearly uncorrelated, $\mbox{TailCoR}^{(j\,k)\,\xi}$ is larger than one as $s_g(\xi,\tau)s(\xi,\tau,\alpha)>1$,\footnote{This is akin to the coefficients of tail dependence steaming from copula theory. For instance, for the bivariate case, the coefficient of tail dependence of a Student-$t$ copula is $2 t_{\alpha+1}\left(-\sqrt{\frac{(\alpha+1)(1-\rho)}{1+\rho}}\right)$, where $t_{\alpha+1}(\cdot)$ is a standardized Student-$t$ cumulative distribution function with tail index $\alpha+1$. Even if $\rho=0$ the tail dependence is positive.} and iii) $\mbox{TailCoR}^{(j\,j)\,\xi}=s_g(\xi,\tau)s(\xi,\tau,\alpha)\sqrt{2}$.

\subsection{Estimation}

Estimation under {\bf G1} -- {\bf G2} is straightforward and  divided in three simple steps.
\begin{description}
\item[Step 1] Standardize $X_{j\,t}$ with the sample median $\hat{\mbox{Q}}^{0.50}_j$ and the sample interquantile range $\hat{\mbox{IQR}}^{\tau}_{j}.$  Likewise for $X_{k\,t}$. Then compute the projection $Z_t^{(j\,k)}$.  
%with the corresponding sample median and IQR, yielding $(\hat{Y}_{j\,t},\hat{Y}_{k\,t})$.
\item[Step 2] Estimate the IQR of the projection: $\hat{\mbox{IQR}}^{(j\,k)\,\xi}_{T}$.
\item[Step 3] Compute the normalization $s_g(\xi,\tau)$ and $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{T}(\hat{\mbox{Q}}^{0.50}_j,\hat{\mbox{Q}}^{0.50}_k,\hat{\mbox{IQR}}^{\tau}_{j},\hat{\mbox{IQR}}^{\tau}_{k}) = s_g(\xi,\tau)\hat{\mbox{IQR}}^{(j\,k)\,\xi}_{T}$.\footnote{This somehow cumbersome notation emphasises that TailCoR is a function of estimated quantiles (step 1)}

%\sladja{Note, we use the notation $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{T}\sladja{(\hat{\mbox{Q}}^{0.50}_j,\hat{\mbox{Q}}^{0.50}_k,\hat{\mbox{IQR}}^{\tau}_{j},\hat{\mbox{IQR}}^{\tau}_{k})}$ to emphasize that $X_{j\,t}$ and $X_{k\,t}$ were standardized with the estimated, not with the theoretical values.}
%In practice $\xi$ takes a limited number of large values, $\xi=\{0.90, 0.95, 0.975, 0.99\}$ say, for which, if $\tau=0.75$, $s_g(\xi,0.75)$ equals 0.526, 0.410, 0.344, and 0.290 respectively.
%\item[Step 4] Compute $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{\hat{Z},T} = s_g(\xi,\tau)\hat{\mbox{IQR}}^{(j\,k)\,\xi}_{\hat{Z},T}$.
\end{description}

%$\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{\hat{Z}\,T}$ is sub-indexed by $\hat{Z}$ and $T$ to explicitly emphasize its dependence with the estimations on steps 1 and 2.
%%The first estimation is the standardization, and hence the hat on $Z$, and the second is the interquantile range of the projection, and hence the hat on $\mbox{IQR}^{(j\,k)\,\xi}$.
%This double source of uncertainty affects the limiting distribution through the variance-covariance matrix, as shown below. 

Under {\bf E1} -- {\bf E5} the linear correlation $\rho_{j\,k}$ is estimated with a robust method. \cite{LindskogMcNeilSchmock03} introduce a robust estimator that is invariant in the class of elliptical distributions. Let $\hat{\kappa}_{j\,k,T}$ be the estimator of  Kendall's correlation.
%{\color{red} I had the feeling that we usually talked about the Pearson correlation?}.
%\begin{equation*}
%\hat{\kappa}_{j\,k,T} = \binom{T}{2}^{-1}\sum_{1\leq t<s\leq T}\mbox{sign}((\hat{X}_{j\,t}-\hat{X}_{j\,s})(\hat{X}_{k\,t}-\hat{X}_{k\,s})).
%\end{equation*}
Then
\begin{equation*}
\hat{\rho}_{j\,k,T} = \sin \left(\frac{\pi}{2}\hat{\kappa}_{j\,k,T} \right),
\end{equation*}
and $\sqrt{1+|\hat{\rho}_{j\,k,T}|}$ follows. Given the $\hat{\mbox{IQR}}^{(j\,k)\,\xi}_{T}$ obtained in step 2 above, the estimator of the nonlinear component is
\begin{equation*}
\hat{s}(\xi,\tau,\alpha)_T = \frac{\hat{\mbox{IQR}}^{(j\,k)\,\xi}_{T}}{\sqrt{1+|\hat{\rho}_{j\,k,T}|}}.
\end{equation*}
%\item[Step 3] Average the nonlinear component for all the pairs
%\begin{equation*}
%\hat{s(\xi,\tau,\alpha)}_{T} = \frac{2}{N(N+1)}\sum_{h=1}^{\frac{N(N+1)}{2}} \hat{s(\xi,\tau,\alpha)}^{(j\,k)}_{h \,T}.
%\end{equation*}

We now see the computational advantages of $\mbox{TailCoR}^{(j\,k)\,\xi}$.
%{\color{red} I wonder if we should not write here rather the estimated version}
It can be estimated exactly for any probability level $\xi$
%This is in contrast with measures based on tail dependence that are asymptotic results.
%Second, $\mbox{TailCoR}^{(j\,k)\,\xi}$ can be computed under the general assumptions {\bf G1}-{\bf G2}, i.e. it is distribution free.
and no optimizations are needed, as it is based on simple steps each requiring a few lines of programming code. This makes $\mbox{TailCoR}^{(j\,k)\,\xi}$ fast to compute.
%and is in contrast with the coefficients of tail dependence steaming from copula theory.
Moreover, estimation of the tail index is not required.
%Though it is assumed to exist under {\bf E1}-{\bf E5}, its estimation is not needed.

%Let $\mbox{\bf Q}^{\tau} =(\mbox{Q}^{0.50}_{j},\mbox{Q}^{\tau}_{j},\mbox{Q}^{0.50}_{k},\mbox{Q}^{\tau}_{k})$ be the vector of quantiles that we use in the standardization \eqref{eq:stand},
%%. We denote by $Cov(\hat{\mbox{\bf Q}}_T^{\tau})$ its variance-covariance matrix,
%and $\hat{\mbox{\bf Q}}^{\tau}_T$ the sample counterpart.\footnote{Note that under ellipticity $\hat{\mbox{Q}}^{\tau}_j=-\hat{\mbox{Q}}^{1-\tau}_j$}
The following theorem shows the consistency of $\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{T}$.
 
 
 
 
\begin{description}
\item[{\bf Theorem 2}]
Let $X_{j\,t}$ and $X_{k\,t}$ be two elements of the random vector $\mathbf{X}_t$ that fulfills assumptions {\bf G1} -- {\bf G2}. Then, as $T \rightarrow \infty$ 
 \begin{equation*}
     \hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{T}(\hat{\mbox{Q}}^{0.50}_j,\hat{\mbox{Q}}^{0.50}_k,\hat{\mbox{IQR}}^{\tau}_{j},\hat{\mbox{IQR}}^{\tau}_{k}) - \mbox{TailCoR}^{(j\,k)\,\xi}=o_p(1).
 \end{equation*}
\end{description}
\begin{description}
\item[{\bf Proof}] See Appendix P.
\end{description}

Next, we prove asymptotic normality. Admittedly, the theorem ignores the effect of the estimated median and the IQR in the standardization of $X_{j\,t}$ and $X_{k\,t}$ (step 1). Monte Carlo results shown below indicate that the effect of step 1 is negligible. 
 
\begin{description}
\item[{\bf Theorem 3}] Let $X_{j\,t}$ and $X_{k\,t}$ be two elements of the random vector $\mathbf{X}_t$ that fulfills assumptions {\bf E1} -- {\bf E5}. Let $f_{(j\,k)}(\cdot)$ and $F_{(j\,k)}(\cdot)$ be the probability density and cumulative distribution functions of $Z^{(j\,k)}_t$, and let $I_{\{\cdot\}}$ be an indicator function that takes value 1 if its argument is true. Then, as $T \rightarrow \infty$
\begin{equation*}
\sqrt{T}\left(\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{T}(\mbox{Q}^{0.50}_j,\mbox{Q}^{0.50}_k,\mbox{IQR}^{\tau}_{j},\mbox{IQR}^{\tau}_{k}) - \mbox{TailCoR}^{(j\,k)\,\xi}\right) \rightarrow_d \mathcal{N}\left(0,4s_g(\xi,\tau)^2\frac{\Gamma(Q^{(j\,k)\xi})}{f^2_{(j\,k)}(F^{-1}_{(j\,k)}(\xi))}\right),
\end{equation*}
where
\begin{eqnarray*}
\Gamma(Q^{(j\,k)\xi}) &=& \sum_{t=-\infty}^{+\infty} {\rm E}\left(W_0(Q^{(j\,k)\xi})W_t(Q^{(j\,k)\xi})\right), \\\\ 
W_t(Q^{(j\,k)\xi}) &=& I_{\{Z^{(j\,k)}_t \leq Q^{(j\,k)\xi}\}}-P(Z^{(j\,k)}_t \leq Q^{(j\,k)\xi}),
%, \mbox{ and} \vspace{0.2cm}\\\\
%\omega &=& \frac{\partial \mbox{Q}^{(j\,k)\,\xi}(\mbox{\bf Q}^{\tau})}{\partial \mbox{\bf Q}^{\tau}}Cov(\hat{\mbox{\bf Q}}_T^{\tau})\frac{\partial \mbox{Q}^{(j\,k)\,\xi}(\mbox{\bf Q}^{\tau})}{\partial \mbox{\bf Q}^{\tau\,'}}.
\end{eqnarray*}
and $\rightarrow_d$ stands for convergence in distribution.
\end{description}

\begin{description}
\item[{\bf Proof}] See Appendix P.
\end{description}

We make the following remarks about the theorem. First, the univariate density $f_{(j\,k)}(\cdot)$ in the denominator is symmetric,
%{\color{red} "elliptical univariate density" does not exist, do we mean "radial function of an elliptical distribution?}
and therefore easy to compute. Second, $\Gamma(Q^{(j\,k)\xi})$ is the long-run component of the variance that accounts for the time dependence.
%Third, it is possible to skip {\bf E3} and derive the elliptical representation of TailCoR without moments. Then $\rho_{j\,k}$ becomes the $(j\,k)$ element of the standardized dispersion matrix that can be estimated with the Tyler's M-estimator (\cite{Tyler87}){\color{red} such an announcement is non-trivial and would require a proof. Not sure if we wish to do that. Have simulations been run to check the validity?}.
Third, the asymptotic variance can be computed by bootstrap, as we do in the empirical application (we use block bootstrap of length 50 and 500 replications). Last, it is possible to derive an equivalent asymptotic distribution under {\bf G1} -- {\bf G2},
%The limiting distribution is more involving since $\hat{\mbox{Q}}^{\tau}_j$ is not necessarily equal to $-\hat{\mbox{Q}}^{1-\tau}_j$,
as shown in the following corollary.  

\begin{description}
\item[{\bf Corollary 1}]
Let $X_{j\,t}$ and $X_{k\,t}$ be two elements of the random vector $\mathbf{X}_t$ that fulfills assumptions {\bf G1} -- {\bf G2}. Let $f_{(j\,k)}(\cdot)$ and $F_{(j\,k)}(\cdot)$ be the probability density and cumulative distribution functions of $Z^{(j\,k)}_t$, and let $I_{\{\cdot\}}$ be an indicator function that takes value 1 if its argument is true. Then, as $T \rightarrow \infty$
\begin{equation*}
\sqrt{T}\left(\hat{\mbox{TailCoR}}^{(j\,k)\,\xi}_{T}(\mbox{Q}^{0.50}_j,\mbox{Q}^{0.50}_k,\mbox{IQR}^{\tau}_{j},\mbox{IQR}^{\tau}_{k}) - \mbox{TailCoR}^{(j\,k)\,\xi}\right) \rightarrow_d \mathcal{N}\left(0,s_g(\xi,\tau)^2\Upsilon\right),
\end{equation*}
where 
\begin{eqnarray*}
&&\Upsilon = 
\frac{\Gamma(Q^{(j\,k)\xi})}{f^2_{(j\,k)}(F^{-1}_{(j\,k)}(\xi))} + \frac{\Gamma(Q^{(j\,k)1-\xi})}{f^2_{(j\,k)}(F^{-1}_{(j\,k)}(1-\xi))} - 2 \frac{\Gamma(Q^{(j\,k)\xi},Q^{(j\,k)1-\xi})}{f_{(j\,k)}(F^{-1}_{(j\,k)}(\xi))f_{(j\,k)}(F^{-1}_{(j\,k)}(1-\xi))}, \vspace{0.2cm}\\\\
&&\Gamma(Q^{(j\,k)\xi},Q^{(j\,k)1-\xi}) = \sum_{t=-\infty}^{+\infty} {\rm E}\left(W_0(Q^{(j\,k)\xi})W_t(Q^{(j\,k)1-\xi})\right), \mbox{ and } \\\\
&& W_t(Q^{(j\,k)\xi}) = I_{\{Z^{(j\,k)}_t \leq Q^{(j\,k)\xi}\}}-P(Z^{(j\,k)}_t \leq Q^{(j\,k)\xi}).
\end{eqnarray*}
%{\color{red} hmmm... don't we get 0 here? I get 2-2. Or should it be an addition? That would give us the 4.}
\end{description}

\begin{description}
\item[{\bf Proof}] If follows from the proof of Theorem 3 but with $Q^{(j\,k)\xi} \neq - Q^{(j\,k)1-\xi}$.
\end{description}

%The univariate densities $f_{(j\,k)}(\cdot)$ are estimated using the \cite{HendricksKoenker92} sandwich form. See the appendix of \cite{CoroneoVeredas12} for a detailed step-by-step implementation.

\subsection{Multivariate TailCoR}

So far we only considered the pair $(j\,k)$ of random variables while the random vector $\mathbf{X}_t$ is of dimension $N$. Considering all the pairs leads to a $N \times N$ symmetric matrix of TailCoRs (including TailCoR of a random variable with itself). For the ease of exposition let $\tilde{N}=N(N+1)/2$. We denote by $\xi_{(j\,k)}$ the probability level at which we compute the IQR for the $(j\,k)$ projection (that is chosen optimally as explained earlier). We assume $\xi_{(j\,k)}=\xi$ $\forall j,k$. This assumption can be easily relaxed, at the expense of notation. 

\begin{description}
\item[{\bf Definition 2}] Under {\bf G1}-{\bf G2}, the matrix of TailCoRs is defined as follows
\begin{equation}\label{eq:vectortailcor}
\mbox{\bf TailCoR}^{\xi} := s_0(\xi,\tau)\mbox{\bf IQR}^{\xi},
\end{equation}
where $\mbox{\bf IQR}^{\xi}$ is a matrix of IQRs of the $N \times N$ projections.
\end{description}

%The assumption $\xi_{(j\,k)}=\xi$ $\forall j,k$ is a simplification that allows definition (\ref{eq:vectortailcor}), but it is possible to relax it at the expense of notation.
Under {\bf E1} -- {\bf E5}, (\ref{eq:vectortailcor}) becomes
\begin{equation}\label{eq:vectortailcorellip}
\mbox{\bf TailCoR}^{\xi} = \sqrt{2}s_g(\xi,\tau)s(\xi,\tau,\alpha)\mathbf \Psi,
\end{equation}
where the matrix $\mathbf \Psi$ has $(j\,k)$ element $\sqrt{\frac{1+|\rho_{j\,k}|}{2}}$. This matrix is symmetric, with unitary diagonal elements, and off-diagonal elements bounded above and below by 1 and $\sqrt{1/2}$ respectively.
%{\color{red} this is now probably no longer true for light-tailed distributions}
It is invariant to location-scale shifts of $\mathbf{X}_t$, and positive definite.
%, and the minimum eigenvalue is 0 and the maximum is bounded by $N$, as their sum equals $N$ (the trace of $\mathbf \Psi$).

Estimation follows the same steps as in the univariate case under {\bf G1} -- {\bf G2}: $\hat{\mbox{\bf TailCoR}}^{\xi}_{T} = s_g(\xi,\tau)\hat{\mbox{\bf IQR}}^{\xi}$. Under {\bf E1} -- {\bf E5}, a new step is added, as $s(\xi,\tau,\alpha)$ is the same for all pairs. Let us rewrite $\hat{s}(\xi,\tau,\alpha)^{(j\,k) \, T}$ in terms of its $\tilde{N}$  components as $\hat{s}(\xi,\tau,\alpha)_{h , T}$, $h=1,\ldots,\tilde{N}$. The nonlinear correlation is estimated by pooling the pairwise estimators:
%{\color{red} wait... we just wrote that, for every $h$, $\hat{s}(\xi,\tau,\alpha)_{h , T}$ would be the same. So in the next sum we take the average of always the same quantity... this makes little sense :-)}
\begin{equation*}
\hat{s}(\xi,\tau,\alpha)_{T} = \frac{1}{\tilde{N}}\sum_{h=1}^{\tilde{N}} \hat{s}(\xi,\tau,\alpha)_{h ,T}.
\end{equation*}
Estimating tail indices by cross-sectionally averaging can be found in, for instance, \cite{Nolan10} and \cite{DominicyOgataVeredas12}.

The asymptotic distribution requires the use of results in \cite{DominicyHormannOgataVeredas12} on covariances between the sample quantiles of marginal distributions under S-mixing.
%Let $\mathbf{Z}_t=(Z^{(1\,1)}_t,\ldots,Z^{(N-1\,N)}_t)=(Z_{1\,t},\ldots,Z_{\tilde{N}\,t})$ be the vector of projections.
%Let $\mathbf{Q}^{\xi}=(Q_{1}^{\xi},\ldots,Q_{\tilde{N}}^{\xi})$ be the vector of quantiles and $\hat{\mathbf{Q}}^{\xi}_T$ the sample counterparts.
%Under {\bf G1}-{\bf G2}, \cite{DominicyHormannOgataVeredas12} show that $\sqrt{T}(\hat{\mathbf{Q}}^{\xi}-\mathbf{Q}^{\xi})\rightarrow \mathcal{N}(\mathbf{0},\bm\Omega)$ where
%Let $\mbox{\bf Q}^{\tau} =(\mbox{Q}^{0.50}_{1},\mbox{Q}^{\tau}_{1},\ldots,\mbox{Q}^{0.50}_{N},\mbox{Q}^{\tau}_{N})$ be the vector of quantiles used in the standardizations of $\mathbf{X}_t$,
%. We denote by $Cov(\hat{\mbox{\bf Q}}^{\tau}_T)$ its variance-covariance matrix,
%and $\hat{\mbox{\bf Q}}^{\tau}_T$ the sample counterpart.
The following theorem shows the asymptotic distribution of the vectorized $\hat{\mbox{\bf TailCoR}}^{\xi}_{T}$.

\begin{description}
\item[{\bf Theorem 4}] 
Let $\mathbf{X}_t$ be a random vector that fulfills assumptions {\bf E1} -- {\bf E5}. 
%\newline
Let
$$vech \hat{\mbox{\bf TailCoR}}^{\xi}_{T}(\mbox{\bf Q}^{0.50}_j,\mbox{\bf Q}^{0.50}_k,\mbox{\bf IQR}^{\tau}_{j},\mbox{\bf IQR}^{\tau}_{k})$$
be the $\tilde{N} \times 1$ half-vectorized matrix of $\hat{\mbox{\bf TailCoR}}^{\xi}_{T}(\mbox{\bf Q}^{0.50}_j,\mbox{\bf Q}^{0.50}_k,\mbox{\bf IQR}^{\tau}_{j},\mbox{\bf IQR}^{\tau}_{k})$. Likewise for $vech \mbox{\bf TailCoR}^{\xi}$. Let $f_{j}(\cdot)$ and $F_{j}(\cdot)$ be the probability density and cumulative distribution functions of the $j$th projection ($j=1,\ldots,\tilde{N}$), and let $I_{\{\cdot\}}$ be an indicator function that takes value 1 if its argument is true. Then, as $T \rightarrow \infty$
\begin{equation*}
\sqrt{T}\left(vech \hat{\mbox{\bf TailCoR}}^{\xi}_{T}(\mbox{\bf Q}^{0.50}_j,\mbox{\bf Q}^{0.50}_k,\mbox{\bf IQR}^{\tau}_{j},\mbox{\bf IQR}^{\tau}_{k}) - vech \mbox{\bf TailCoR}^{\xi}\right) \rightarrow_d \mathcal{N}\left(0,4s_g(\xi,\tau)^2\bm\Omega\right),
\end{equation*}
where $\bm\Omega$ is a $N \times N$ matrix with $(j\,j)$ element
\begin{eqnarray*}
\Omega_{j\,j} &=& \frac{\Gamma_{j\,j}(Q^{\xi}_j)}{f^2_j(F_j^{-1}(\xi))}, \mbox{ where} \\
\Gamma_{j\,j}(Q^{\xi}_j) = \sum_{t=-\infty}^{\infty} {\rm E}(W_0(Q^{\xi}_j),W_t(Q^{\xi}_j)) &\mbox{ and }& W_t(Q^{\xi}_j) = I_{\{Z_{j\,t} \leq Q^{\xi}_j \}} - P(Z_{j\,t} \leq Q^{\xi}_j).
\end{eqnarray*}
The $(j\,k)$ element of $\bm\Omega$ is
\begin{eqnarray*}
\Omega_{j\,k} &=& \frac{\Gamma_{j\,k}(Q^{\xi}_j,Q^{\xi}_k)}{f_j(F_j^{-1}(\xi))f_k(F_k^{-1}(\xi))} \forall j \neq k, \mbox{ where} \\
\Gamma_{j\,k}(Q^{\xi}_j) &=& \sum_{t=-\infty}^{\infty} {\rm E}(W_0(Q^{\xi}_j,Q^{\xi}_k),W_t(Q^{\xi}_j,Q^{\xi}_k)) \mbox{ and }\\
W_t(Q^{\xi}_j,Q^{\xi}_k) &=& I_{\{Z_{j\,t} \leq Q^{\xi}_j,Z_{k\,t} \leq Q^{\xi}_k \}} - P(Z_{j\,t} \leq Q^{\xi}, Z_{k\,t} \leq Q^{\xi}_k).
\end{eqnarray*}
%and
%\begin{equation*}
%\bm\omega = \frac{\partial \mbox{\bf Q}^{\xi}(\mbox{\bf Q}^{\tau})}{\partial \mbox{\bf Q}^{\tau}}Cov(\hat{\mbox{\bf Q}}^{\tau}_T)\frac{\partial \mbox{\bf Q}^{\xi}(\mbox{\bf Q}^{\tau})}{\partial \mbox{\bf Q}^{\tau \,'}}.
%\end{equation*}
\end{description}

\begin{description}
\item[{\bf Proof}] See Appendix P.
\end{description}



==> RV_MonteCarlo_JoE.tex <==
\section{A Monte Carlo simulation study}

We analyze the finite sample properties of TailCoR with three bivariate elliptical distributions: Gaussian, Student-$t$ with $\alpha=2.5$, and ES with $\alpha=1.5$. The most heavy tailed distribution is the Student-$t$, followed by the ES and the Gaussian. The location parameters are set to zero and the dispersion matrix has unitary diagonal elements and off-diagonal elements $0.50$. We consider three sample sizes $T=\{1000, 5000, 10000\}$ and two replication sizes $H=\{1000,10000\}$. In the sequel we show results for $T=10000$ and $H=10000$, unless otherwise stated. Results for other configurations are alike and they are available upon request.

%\begin{center}[FIGURE \ref{fig:distributions} ABOUT HERE]\end{center}

\begin{figure}
  \begin{center}\caption{TailCoR for different distributions} 
\includegraphics[angle=0,width=0.6\linewidth]{GaussianStudentTES.eps}\label{fig:distributions}
\begin{tabular}{p{9cm}} 
\scriptsize Distribution of 10000 estimated TailCoR's for $\xi=0.95$ and three distributions: Gaussian (solid line), Student-$t$ with $\alpha=2.5$ (dashed line), ES with $\alpha=1.5$ (dotted line).\\ 
\end{tabular}
  \end{center}
\end{figure}


Figure \ref{fig:distributions} shows the finite sample distributions of the TailCoR estimates for $\xi=0.95$ and for the three distributions (solid line for the Gaussian, dashed for the Student-$t$, and dotted for the ES). In all cases, TailCoR is larger than one. The estimated TailCoR is more precise under Gaussianity than under heavy tails, as it only depends on the linear correlation. Moreover, the median is around 1.22, very close to the true value $\sqrt{1+0.50}=1.225$. Estimates under the Student-$t$ and the ES have higher medians (1.58 for the ES and 1.64 for the Student-$t$), reflecting the nonlinear dependencies.
% and are more dispersed, reflecting the effect of the tail index.

%\begin{figure}
%  \begin{center}\caption{TailCoR for different distributions} 
%\includegraphics[angle=0,width=0.6\linewidth]{Overlapplot.pdf}\label{fig:distributions}
%\begin{tabular}{p{9cm}} 
%\scriptsize Distribution of 500 estimated TailCoR for $\xi=0.95$ and three distributions: Gaussian (solid line), Student-$t$ with $\alpha=2.5$ (dashed line) and ES with $\alpha=1.5$ (dotted line).\\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%\begin{center}[FIGURE \ref{fig:xi} ABOUT HERE]\end{center}

\begin{figure}
  \caption{Sensitivity of TailCoR to $\xi$}\label{fig:xi}
  \begin{center}
    \subfloat[Gaussian]{\includegraphics[angle=0,width=.35\linewidth]{Gaussian09095099.eps}}
    \subfloat[Student-$t$]{\includegraphics[angle=0,width=.35\linewidth]{Student09095099.eps}}\\
    \subfloat[ES]{\includegraphics[angle=0,width=.35\linewidth]{ES09095099.eps}} \\
\begin{tabular}{p{11cm}}
\scriptsize Sensitivity of TailCoR to $\xi$ for the Gaussian (panel a), Student-$t$ with $\alpha=2.5$ (panel b), and ES with $\alpha=1.5$ (panel c) distributions. Each line is the density of the 10000 estimates of TailCoR for different values of $\xi$: 0.90 (solid line), 0.95 (dashed) and 0.99 (dotted).\\ 
\end{tabular}
  \end{center}
\end{figure}

Figure \ref{fig:xi} shows the sensitivity of TailCoR to $\xi$ for the Gaussian (panel (a)), Student-$t$ with $\alpha=2.5$ (panel (b)), and ES with $\alpha=1.5$ (panel (c)). Solid lines are for $\xi=0.90$, dashed for $\xi=0.95$, and dotted for $\xi=0.99$.
%Each line is the density of the 10000 estimates of TailCoR for different values of $\xi$: 0.90 (solid line), 0.95 (dashed) and 0.99 (dotted).
The densities overlap for the Gaussian distribution since $\mbox{TailCoR}^{(j\,k)\,\xi}$ does not depend on $\xi$ (it equals $\sqrt{1+|\rho_{j\,k}|}$).
%{\color{red} then why is there no complete overlap? I do see various densities at the same center... a mistake?}
The small differences are due to finite sample discrepancies. Regarding the other distributions, results show that, as expected, TailCoR increases with $\xi$.

%\begin{figure}[!h]
%  \caption{Sensitivity of TailCoR to $\xi$}\label{fig:xi}
%  \begin{center}
%    \subfloat[Gaussian]{\includegraphics[angle=0,width=.35\linewidth]{tailcorGauschangexi}} \\
%    \subfloat[Student-$t$]{\includegraphics[angle=0,width=.35\linewidth]{tailcorstudentchangexi}}
%    \subfloat[ES]{\includegraphics[angle=0,width=.35\linewidth]{tailcorESchangexi}} \\
%\begin{tabular}{p{11cm}}
%\scriptsize Sensitivity of TailCoR to $\xi$ for the Gaussian (top plot), Student-$t$ with $\alpha=2.5$ (bottom left plot) and ES with $\alpha=1.5$ (bottom right plot). Each line is the density of the 500 estimates of TailCoR for different values of $\xi$: 0.90 (solid line), 0.95 (dashed) and 0.99 (dotted).\\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%\begin{center}[FIGURE \ref{fig:linear} ABOUT HERE]\end{center}
%
%Figure \ref{fig:linear} shows the density of the estimates of $\sqrt{1+\rho_{j\,k}}$ for $\xi=0.95$ and for the three distributions (solid line for the Gaussian, dashed for the Student-$t$, and dotted for the ES). If estimated correctly, they should be invariant to the tail thickness. Indeed, the median of the estimates for the three distributions are very close to the true value $1.225$, with a slight bias for the Gaussian, and the precision decreases with the tail thickness.

%\begin{figure}
%  \begin{center} \caption{The linear component}
%%\vspace{-3.5cm}
%%    \subfigure[TailCoR for different distributions]{\includegraphics[angle=0,width=0.8\linewidth]{nonlineardistrib.pdf}}
%\includegraphics[angle=0,width=0.6\linewidth]{linearcompdistrb}\label{fig:linear}
%\begin{tabular}{p{9cm}}
%\scriptsize Density of the 500 estimates of $\sqrt{1+\rho_{j\,k}}$ for $\xi=0.95$ and for the three distributions (solid line for the Gaussian, dashed for the Student-$t$, and dotted for the ES). \\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%\begin{center}[FIGURE \ref{fig:KDE} ABOUT HERE]\end{center}

\begin{figure}
  \caption{Convergence in distribution}\label{fig:KDE}
  \begin{center}
    \subfloat{\includegraphics[angle=0,height =5cm,width=.30\linewidth]{ConvDist10001000.eps}}
    \subfloat{\includegraphics[angle=0,height =5cm,width=.30\linewidth]{ConvDist50001000.eps}}
    \subfloat{\includegraphics[angle=0,height =5cm,width=.30\linewidth]{ConvDist100001000.eps}}\\
    \subfloat{\includegraphics[angle=0,height =5cm,width=.30\linewidth]{ConvDist100010000.eps}} 
    \subfloat{\includegraphics[angle=0,height =5cm,width=.30\linewidth]{ConvDist500010000.eps}} 
    \subfloat{\includegraphics[angle=0,height =5cm,width=.30\linewidth]{ConvDist1000010000.eps}} \\
\begin{tabular}{p{13cm}}
\scriptsize Kernel densities (red line)  of the centered estimates against a corresponding Gaussian distribution (black line) for all the combinations of the sample size and replications (indicated in the top of each plot).\\ 
\end{tabular}
  \end{center}
\end{figure}

The precision and convergence in distribution of the estimator are shown in Figure \ref{fig:KDE} and in Table \ref{tab:step1}  for $\xi=0.95$. Red lines in the figure are the kernel densities of the centered estimates for different sample sizes and replications (indicated at the top of each plot), and the black lines are the corresponding Gaussians. As expected, the kernel densities approach to the limiting distribution as the sample size and the number of replications increase. The table shows the effect of the estimation error of step 1. It compares TailCoR and its components when the population and the sample quantiles are used in step 1 (as shown in the row "Step 1"). Estimations are done for the Gaussian and Student-$t$ distributions, two sample sizes (1000 and 10000), 1000 replications, and $\xi=0.95$. Mean estimates are very close to the true values, indicating unbiasedness. The standard errors are very small and, more importantly, using the sample quantiles in step 1 does not affect significantly the accuracy of the estimates in step 2.

%The smooth line in the figure is the standardized Gaussian while the bars are the histograms of the standardized estimates for different sample sizes and replications (indicated at the top of each plot). As expected, the histograms approach to the limiting distribution as the sample size and the replications increase.


%\begin{table}
%\begin{center}
%\caption{Mean and variances} \label{tab:meanvarMC}
%\begin{tabular}{cccc}
% \hline\hline
%$T$ & $H$ & Mean & Variance \\ \hline
%1000&1000&1.63&0.077\\
%1000&10000& 1.64&0.076\\
%5000&1000& 1.64&0.035\\
%5000&10000&1.64&0.034\\
%10000&1000&1.64&0.024\\
%10000&10000&1.64&0.024\\ \hline \hline
%\multicolumn{4}{p{5cm}}{\footnotesize{Mean and variances of the TailCoR estimates and for all the combinations of the sample size and replications.}}
%\end{tabular}
%\end{center}
%\end{table}


%Last, since assumptions {\bf G1} and {\bf E4} allow for time dependencies, we also run a Monte Carlo study with a bivariate CCC -- constant conditional correlation -- model with Student-$t$ innovations. Results, available under request, indicate that the finite sample distribution of the estimated TailCoR is unimodal, similar to those shown here, but the average TailCoR increases with the degree of dependence in the variance-covariance matrix.

%\begin{figure}
%  \begin{center} \caption{Convergence in distribution}
%\vspace{0.2cm}
%\includegraphics[angle=0,width=0.6\linewidth]{histconvergence}\label{fig:hist}
%\begin{tabular}{p{9cm}}
%\scriptsize Histogram of $\sqrt{T}\left(\hat{\mbox{TailCoR}}^{0.95}_{\hat{Z}\,T} - \mbox{TailCoR}^{0.95}\right)$ as a function of the number of observations and replications (indicated in the top of each plot) against the standardized Gaussian distribution.\\ 
%\end{tabular}
%  \end{center}
%\end{figure}

%{\bf Show the losses by ignoring the parameter uncertainty}

\begin{table}
\begin{center}
\caption{Estimation uncertainty step 1} \label{tab:step1}
\begin{tabular}{lccccc}
\hline\hline
Step 1:          &                  & Popul.       & Sample             & Popul.          & Sample\\
\hline
& & \multicolumn{2}{c}{Gaussian} & \multicolumn{2}{c}{Student-$t$} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & \multicolumn{4}{c}{TailCoR} \\
                     & True          & 1.225         &  1.225        &     1.637      &    1.637   \\
$T=1000$     & Mean         & 1.223         &  1.224        &    1.639       &   1.635    \\
                     & SD                   &  0.034        &  0.037       &      0.082     & 0.077   \\
$T=10000$   & Mean         & 1.225         &  1.225       &     1.637      &     1.637  \\
                     & SD                   &  0.011        &  0.011       &     0.024       &   0.024  \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & \multicolumn{4}{c}{$s(\xi,\tau,\alpha)$} \\
                     & True          & 2.438         &  2.438        &     3.259      &    3.259    \\
$T=1000$     & Mean         & 2.435         &  2.438        &   3.266        &    3.257   \\
                     & SD                   & 0.059         &  0.072       &      0.152     & 0.147  \\
$T=10000$   & Mean         & 2.439         &  2.438        &    3.260       &     3.259  \\
                     & SD                   & 0.020         &  0.023       &      0.045      &   0.046   \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & \multicolumn{4}{c}{$\sqrt{1+|\rho_{j\,k}|}$} \\
                     & True          & 1.225         &  1.225        &     1.225      &  1.225     \\
$T=1000$     & Mean         & 1.225         &  1.224        &     1.224      &     1.224  \\
                     & SD                   &  0.011        &  0.011       &      0.012      &0.012    \\
$T=10000$   & Mean         & 1.225         &  1.225        &     1.224      &    1.225   \\
                     & SD                 &  0.003        &  0.003        &        0.004      &   0.004  \\
\hline \hline
\multicolumn{6}{p{10cm}}{\footnotesize{Means and standard deviations of estimates of TailCoR and its components when using population (Popul. in top row) or sample marginal quantiles in step 1. All results are for H=1000 and $\xi=0.95$}}
\end{tabular}
\end{center}
\end{table}


